The Power of Pivoting for Exact Clique Counting

Clique counting is a fundamental task in network analysis, and even the simplest setting of $3$-cliques (triangles) has been the center of much recent research. Getting the count of $k$-cliques for larger $k$ is algorithmically challenging, due to the exponential blowup in the search space of large cliques. But a number of recent applications (especially for community detection or clustering) use larger clique counts. Moreover, one often desires \textit{local} counts, the number of $k$-cliques per vertex/edge. Our main result is Pivoter, an algorithm that exactly counts the number of $k$-cliques, \textit{for all values of $k$}. It is surprisingly effective in practice, and is able to get clique counts of graphs that were beyond the reach of previous work. For example, Pivoter gets all clique counts in a social network with a 100M edges within two hours on a commodity machine. Previous parallel algorithms do not terminate in days. Pivoter can also feasibly get local per-vertex and per-edge $k$-clique counts (for all $k$) for many public data sets with tens of millions of edges. To the best of our knowledge, this is the first algorithm that achieves such results. The main insight is the construction of a Succinct Clique Tree (SCT) that stores a compressed unique representation of all cliques in an input graph. It is built using a technique called \textit{pivoting}, a classic approach by Bron-Kerbosch to reduce the recursion tree of backtracking algorithms for maximal cliques. Remarkably, the SCT can be built without actually enumerating all cliques, and provides a succinct data structure from which exact clique statistics ($k$-clique counts, local counts) can be read off efficiently.

==> pivoter long for arxiv/algo.tex <==
%ass[../main.tex]{subfiles}
\section{Preliminaries} \label{sec:prelims}

We start with the mathematical formalism required to describe the main
algorithm and associated proofs. The input is a simple, undirected
graph $G = (V,E)$, where $|V| = n$ and $|E| = m$. It is convenient to assume
that $G$ is connected. We use vertices
to denote the elements of $V$ (the term \emph{nodes} will be used for a different construct).
We use the following notation for neighborhoods.

\begin{asparaitem}
    \item $N(v)$: This is the neighborhood of $v$.
    \item $N(S,v)$: For any subset of vertices $S$, we use $N(S,v)$ to denote $N(v) \cap S$.
Alternately, this is the neighborhood of $v$ in $S$.
\end{asparaitem}
%
We will use \emph{degeneracy orderings} (or core decompositions) to reduce
the recursion tree. This is a standard technique for clique counting~\cite{ChNi85,FFF15,JS17,DBS18}.
This ordering is obtained by iteratively removing the minimum degree vertex,
and can be computed in linear time~\cite{MB83}. Typically, one uses this
ordering to convert $G$ into a DAG. The largest \emph{out-degree} is the 
graph degeneracy, denoted $\alpha$. We state this fact as a lemma,
which is considered a classic fact in graph theory and network science.

\begin{lemma} \label{lem:degen}~\cite{MB83} Given a graph $G = (V,E)$, there is a 
linear time algorithm that constructs an ayclic orientation of $G$
such that all outdegrees are at most $\alpha$.
\end{lemma}

The most important construct we design is the \emph{Succinct Clique Tree} (SCT) $\bT$.
% The underlying tree is basically an ``unrolled" version of the BK recursion tree \Shweta{what do we mean by unrolled?}, with further
% degeneracy optimizations as given by ELS. We use the terms \emph{nodes} and \emph{links}
% to refer to the SCT Tree.
The SCT stores special node and link attributes that are key to getting global and local
clique counts, for all values of $k$.
The construction and properties of the SCT are given in the next section. Here, 
we list out technical notation associated with the SCT $\bT$.

Formally, $\bT$ is a tree where nodes are labeled with subsets of $V$, with the following
properties.
\begin{asparaitem}
    \item The root is labeled $V$.
    \item Parent labels are strict supersets of child labels.
    \item Leaves are labeled with the empty set $\emptyset$.
\end{asparaitem}

\medskip

An important aspect of $\bT$ are \emph{link labels}. A link label is a
pair with a vertex of $V$ and a ``call type".
The label is of the form $(v,\mathfrak{p})$ or $(v,\mathfrak{h})$,
where $\mathfrak{p}$ is shorthand for ``pivot" and $\mathfrak{h}$ for ``hold".
For a link label $(v,\cdot)$ of the link $(S,S')$ (where $S \supset S'$ is the parent),
$v$ will be an element of $S$.

Consider a root to leaf path $T$ of $\bT$. We have the following associated
set of vertices. It is convenient to think of $T$ as a set of tree links.

\begin{asparaitem}
    \item $H(T)$: This is the set of vertices associated with ``hold" call types,
    among the links of $T$. Formally, $H(T)$ is
    $\{v | \textrm{$(v,\mathfrak{h})$ is label of link in $T$}\}$.
    \item $P(T)$: This is the set of vertices with ``pivot" calls. Formally $P(T)$ is
    $\{v | \textrm{$(v,\mathfrak{p})$ is label of link in $T$}\}$.
\end{asparaitem}

\medskip

We now describe our algorithm. We stress that the presentation here is different
from the implementation. The following presentation is easier for mathematical
formalization and proving correctness. The implementation is a recursive 
version of the same algorithm, which is more space efficient. This
is explained in the proof of \Thm{main}.

\section{Building the SCT} \label{sec:scr}

We give the algorithm to construct the SCT. 
% This is essentially an explicit construction
% of the BK recursion tree \Shweta{with the added constraint that pivot cannot be from X}, with degeneracy optimization of ELS. 
We keep track
of various attributes to appropriately label the edges.
The algorithm will construct the SCT $\bT$ in a breadth-first manner. Every
time a node is processed, the algorithm creates its children and labels all the new
nodes and links created.

\begin{algorithm}
\caption{\scr($G$) \newline
Output: SCT of $G$ 
}
Find degeneracy orientation of $G$, and let $N^+(v)$ denote the outneighborhood of a vertex $v$.\\
Initialize tree $\bT$ with root labeled $V$.\\
For every $v \in V$, create a child of root with node label $N^+(v)$. Set the 
edge label to $(v,\mathfrak{h})$. \\
Insert all these child nodes into a queue $\bQ$. \\
While $\bQ$ is non-empty: \\
\ \ \ \ Dequeue to get node $\gamma$. Let node label be $S$.\\
\ \ \ \ If $S = \emptyset$, continue. \\
\ \ \ \ Find $p \in S$ with largest $N(S,p)$ value. \label{step:pivot} \\
\ \ \ \ Create child node of $\gamma$ with vertex label $N(S,p)$. Add this node to $\bT$ and set the link
label (of the new link) to $(p,\mathfrak{p})$. Also, add this node to $\bQ$. \label{step:pcall}\\
\ \ \ \ Let $S \setminus (p \cup N(p)) = \{v_1, v_2, \ldots, v_\ell\}$ (listed
in arbitrary order). \\
\ \ \ \ For each $i \leq \ell$: create child node of $\gamma$ labeled
$N(S,v_i) \setminus \{v_1, v_2, \ldots, v_{i-1}\}$. Add this node to $\bT$ and set link label to $(v_i, \mathfrak{h})$.
Also add this node to $\bQ$. \label{step:nncall}\\
Return $\bT$. 
% Declare global hash tables $T_k, T_V, T_E$.  \\
% Order $V$ by degeneracy ordering and convert $G$ into a DAG. For $v\in V$, let $N^+_v$ denote the outneighborhood of $v$. \\
% For $v$ in $V$: \\ \label{step:for-parallel}
% \ \ \ \ $\mainalgrec{(\{v\}, \emptyset, N^+_v)}$ 
\end{algorithm}

As mentioned earlier, the child of the node labeled $S$ has one child corresponding
to the pivot vertex $p$, and children for all non-neighbors of $p$. Importantly,
we label each ``call" with $\mathfrak{p}$ or $\mathfrak{h}$. This is central to getting
unique representations of all the cliques.

Now for our main theorem about SCT.

\begin{theorem} \label{thm:scr} Every clique $C$ (in $G$) can be \emph{uniquely}
represented as $H(T) \cup Q$, where $Q \subseteq P(T)$ and $T$ is a root to leaf path in $\bT$.
(Meaning, for any other root to leaf path $T' \neq T$, $\forall Q \subseteq P(T')$,
$C \neq H(T') \cup Q$.)
\end{theorem}

We emphasize the significance of this theorem. Every root to leaf
path $T$ represents a clique, given by the vertex set $H(T) \cup P(T)$. Every clique $C$ 
is a subset of potentially many such sets; and there is no obvious bound on this number. So one can think of
$C$ ``occurring" multiple times in the tree $\bT$. But \Thm{scr} asserts that 
if we take the labels into account ($H(T)$ vs $P(T)$),
then there is a \emph{unique} representation or ``single occurrence" of $C$.

\begin{proof} (of \Thm{scr}) 
Consider a node $\gamma$ of $\bT$ labeled $S$. We prove, by induction on $|S|$,
that every clique $C \subseteq S$ can be expressed as $H(T) \cup Q$,
where $T$ is a path from $\gamma$ to a leaf, and $Q \subseteq P(T)$. The theorem
follows by setting $\gamma$ to the root.

The base case is vacuously tree, since for empty $S$, all relevant sets are empty.
Now for the induction. We will have three cases. Let $p$ be the pivot chosen
in \Step{pivot}. (If $S$ is the root, then there is no pivot. We will directly go
to Case (iii) below.)

{\em Case (i): $p \in C$.} By construction, there is a link labeled $(p,\mathfrak{p})$
to a child of $\gamma$. Denote the child $\beta$.
The child $\beta$ has label $N(S,p)$. Observe that $C \setminus p$
is a clique in $N(S,p)$ (since by assumption, $C$ is a clique in $S$.)
By induction, there is a unique representation 
$C\setminus p = H(T) \cup Q$, for path $T$ from the child node
to a leaf and $Q \subseteq P(T)$. Moreover there cannot be a representation
of $C$ by a path rooted at $\beta$, since $N(S,p) \not\ni p$.
Consider the path $T'$ that contains
$T$ and starts from $\gamma$. Note that $H(T') = H(T)$ and $P(T') = P(T) \cup p$.
We can express $C = H(T') \cup (Q \cup p)$, noting that $Q \cup p \subseteq P(T')$.
This proves the existence of a representation. Moreover, there is only one representation
using a path through $\beta$. 

We need to argue that no other path can represent $C$. The pivoting is critical for this step.
Consider any path rooted at $\gamma$, but not passing through $\beta$.
It must pass through some other child, with corresponding links labeled $(v_i,\mathfrak{h})$,
where $v_i$ is a \emph{non-neighbor} of $p$. Since $C \ni p$, a non-neighbor $v_i$
cannot be in $C$. Moreover, for any path $\hat{T}$ passing through these other children,
$\hat{T}$ must contain some non-neighbor. Thus, $\hat{T}$ cannot represent $C$.

{\em Case (ii): $C \subseteq N(S,p)$.} The argument is essentially identical to the one above.
Note that $C\setminus p = C$, and by induction $C\setminus p$ has a unique representation
using a path through $\beta$. For uniqueness, observe that $C$ does not contain a non-neighbor of $p$.
The previous argument goes through as is.

{\em Case (iii): $C$ contains a non-neighbor of $p$.} Recall that $S \setminus (N(p) \cup p)$
(the set of non-neighbors in $S$) is denoted $\{v_1, v_2, \ldots, v_\ell\}$. Let $i$
be the smallest index $i$ such that $v_i \in C$. For any $1 \leq j \leq \ell$, let
$N_j := N(S,v_j) \setminus \{v_1, v_2, \ldots, v_{j-1}\}$. Observe that for all $j$,
there is a child labeled $N_j$. Moreover, all the link labels have $\mathfrak{h}$,
so for path $T$ passing through $N_j$, $H(T) \ni v_j$. Thus, if $T$ can represent $C$,
it cannot pass through $N_j$ for $j < i$. Moreover, if $j > i$, then $N_j \not\ni v_i$
and no path passing through this node can represent $C$.

Hence, if there is a path that can represent $C$, it must pass through $N_i$.
Note that $C\setminus v_i$ is a clique contained in $N_i$. By induction,
there is a unique path $T$ rooted at $N_i$ such that $C \setminus v_i = H(T) \cup Q$,
for $Q \subseteq P(T)$. Let $T'$ be the path that extends $T$ to $\gamma$.
Note that $H(T') = H(T) \cup v_i$, so $C = H(T') \cup Q$. The uniqueness of $T$
implies the uniquesness of $T'$.
% 
% For any path rooted at $\gamma$
% passing through the child labeled $N(S,v_j) \setm
% 
% 
% 
% 
% Suppose there existed a path (rooted at $\gamma$) $\hat{T} \neq T'$ and $\hat{Q} \subseteq P(\hat{T})$
% such that $C = H(\hat{T}) \cup \hat{Q}$. This path passes through some child of $\gamma$.
% Suppose that child is $\beta$, and let the portion of $\hat{T}$ rooted at $\beta$
% be denoted $\widetilde{T}$. Since the label of $\beta$ is $N(S,p)$, 
% $L(\widetilde{T})$ cannot contain $p$. Thus, $\widetilde{T}$ must have a representation
% of $C \setminus p$. But by induction, $C \setminus p$ has 
% 
% 
% 
\end{proof}

\section{Getting global and local counts} \label{sec:count}

% The tree $\bT$ is succinct, since it explicitly ``stores" only maximal cliques \Shweta{no, it doesn't}. But one can extract
% fine-grained information about all cliques.

The tree $\bT$ is succinct and yet one can extract fine-grained information from it about all cliques.

\begin{algorithm}
\caption{\mainalg($G$) \newline
Output: Clique counts of $G$
}
Let $\bT = \scr(G)$.\\
Initialize all clique counts to zero.\\
For every root to leaf path $T$ in $\bT$:\\
\ \ \ \ For every $0 \leq i \leq |P(T)|$, increment $C_{|H(T)|+i}$ by ${P(T) \choose i}$.\\
\ \ \ \ For every $v \in H(T)$ and every $0 \leq i \leq |P(T)|$, increment $c_{|H(T)|+i}(v)$
by ${P(T) \choose i}$. \label{step:ht} \\
\ \ \ \ For every $v \in P(T)$ and every $0 \leq i \leq |P(T)|-1$, increment $c_{|H(T)|+i+1}(v)$
by ${{P(T)-1} \choose i}$. \label{step:pt} \\
\ \ \ \ For every edge $e(u,v), u \in H(T), v \in H(T), u \neq v$ and every $0 \leq i \leq |P(T)|$, increment $c_{|H(T)|+i}(e)$
by ${{P(T)} \choose i}$. \label{step:hht} \\
\ \ \ \ For every edge $e(u,v), u \in P(T), v \in H(T)$ and every $0 \leq i \leq |P(T)|-1$, increment $c_{|H(T)|+i+1}(e)$
by ${{P(T)-1} \choose i}$. \label{step:pht} \\
\ \ \ \ For every edge $e(u,v), u \in P(T), v \in P(T), u \neq v$ and every $0 \leq i \leq |P(T)|-2$, increment $c_{|H(T)|+i+2}(e)$
by ${{P(T)-2} \choose i}$. \label{step:ppt} \\
% \ \ \ \ For every $v \in P(T)$ and every $u \in P(T), u \noteq v$, for every $0 \leq i \leq |P(T)|-2$, increment $c_{|H(T)|+i+1}(e)$
% by ${{P(T)-2} \choose i}$. \label{step:pt} \\
% every $0 \leq i \leq |P(T)|-1$, increment $c_{|H(T)|+i+1}(v)$
% by ${{P(T)-1} \choose i}$. \label{step:pt} \\
Output the sets of values $\{C_k\}$, $\{c_k(v)\}$ and $\{c_k(e)\}$.
\end{algorithm}

% One can also get per-edge counts, but there are three cases. We omit that for space
% reasons, and give details in the full version.
% (Per-edge counts can be obtained in $O(\alpha^3 |\sct(G)|)$. Again, this proof
% is in the full version.)

The storage complexity of the algorithm, as given, is potentially $O(\alpha^2 |\sct(G)|)$,
since this is required to store the tree. In the proof of \Thm{main}, we explain how
to reduce the storage.

% \begin{theorem} \label{thm:mainalg} \mainalg{} correctly outputs
% all global and local counts. Furthermore, \mainalg{} runs in time $O(\alpha^2 |\sct(G)|+m)$.
% \end{theorem}

\begin{proof} (of \Thm{main}) {\bf Correctness:} By \Thm{scr}, a root to leaf path $T$ of $\bT$ represents exactly
$2^{P(T)}$ different cliques, with ${P(T) \choose i}$ of size $|H(T)| + i$. Moreover,
over all $T$, this accounts for all cliques in the graph. This proves the correctness
of global counts.

Pick a vertex $v \in H(T)$. For every subset of $P(T)$, we get a different
clique containing $v$ (that is uniquely represented by \Thm{scr}). This 
proves the correctness of \Step{ht}. For a vertex $v \in P(T)$,
we look at all subsets containing $v$. Equivalently, we get a different
represented clique containing $v$ for every subset of $P(T)\setminus v$. This 
proves the correctness of \Step{pt}.

Pick an edge $e=(u,v), u \in H(T), v \in H(T)$. For every subset of $P(T)$, we get a different
clique containing $e$ (that is uniquely represented by \Thm{scr}). This 
proves the correctness of \Step{hht}. For an edge $e=(u,v), u \in P(T), v \in H(T)$,
we look at all subsets of $P(T)$ containing $u$. Equivalently, we get a different
represented clique containing $e$ for every subset of $P(T)\setminus u$. This 
proves the correctness of \Step{pht}. For an edge $e=(u,v), u \in P(T), v \in P(T)$,
we look at all subsets of $P(T)$ containing both $u$ and $v$. Equivalently, we get a different
represented clique containing $e$ for every subset of $P(T)\setminus v \setminus u$. This 
proves the correctness of \Step{ppt}.

{\bf Running time (in terms of $|\sct(G)|$):} Consider the procedure $\scr(G)$. Note that the size of $\bT$
is at least $n$, so we can replace any running time dependence on $n$ by $|\bT|$.
The degeneracy orientation can be found in $O(m+n)$~\cite{MB83}. For the actual building
of the tree, the main cost is in determining the pivot and constructing the children
of a node. Suppose a non-root node labeled $S$ is processed. The above mentioned steps can be done
by constructing the subgraph induced on $S$. This can be done in $O(|S|^2)$ time. Since
this is not a root node, $|S| \leq \alpha$ (this is the main utility of the degeneracy
ordering). Thus, the running time of $\scr(G) = O(\alpha^2|\bT|) = O(\alpha^2 |\sct(G)|)$.

Now we look at \mainalg. Note that the subsequent counting steps do \emph{not}
need the node labels in $\bT$; for all path $T$, one only needs $P(T)$ and $H(T)$.
The paths can be looped over by a DFS from the root. For each path,
there are precisely $|P(T)|+1$ updates to global clique counts,
and at most $|H(T) \cup P(T)| \times (|P(T)|+1)$ updates to per-vertex clique counts.
The length of $T$ is at most $\alpha$, and thus both these quantities
are $O(\alpha^2)$. Thus, the total running time is $O(\alpha^2 |\sct(G)|)$ for global and per-vertex clique counting.

Similarly, for each path, at most $|H(T) \cup P(T)|^2 \times (|P(T)|+1)$ updates are made to per-edge clique counts. This quantity is $O(\alpha^3)$. Thus, the total running time is $O(\alpha^3 |\sct(G)|)$.

% We can bound the running time of $\scr(G)$ (and hence, $|\sct(G)|$) 
% We now try to bound $\sct(G)$. Note that every node enters the queue $Q$ exactly once and is removed from the queue exactly once. Thus, $\sct(G)$ is bounded above by the running time of \scr{}.

% {\bf Running time (fine grained):} 

{\bf Running time (in terms of $n$ and $\alpha$):} One crucial difference between the algorithm of Bron-Kerbosch and \scr{} is that in Bron-Kerbosch, the pivot vertex can be chosen not only from $S$ but also from a set of already processed vertices. Hence, the tree obtained in Bron-Kerbosch can potentially be smaller than that of \mainalg{}. Despite this difference, the recurrence and bound on the worst case running time of $\scr{}$ is the same as Bron-Kerbosch. 
% This gives a finer bound on the running time.

\begin{theorem} \label{thm:main-BK} Worst case running time of \scr{} is $O(n3^{\alpha/3})$. 
\end{theorem}
%%%%%%%%%%%%
%Pivoter obtains the global and per-vertex counts in
% time $O(n3^{\alpha/3})$ and per-edge counts in time
% $O(n\alpha3^{n/3})$. 
\begin{proof}
Let $T(s)$ be the worst case running time required by \scr{} to process $S$ where $s=|S|$.

Let $R=S \setminus N(p)$. Let $T_r(s)$ be the worst case running time of processing $S$ when $|R|=r$. Note that when $S$ is being processed it creates a total of $r$ child nodes. 

Thus, $T(s)=\max\limits_r\{T_r(s)\}$. 

Note that all steps other than \Step{pcall} and \Step{nncall} take time $O(s^2)$. Say, they take time $p_1s^2$, where $p_1>0$ is a constant.

Thus, we have that:
\begin{align}
    T_r(s) \leq \sum\limits_{v \in R}{T(|N(S,v)|) 
    + p_1s^2}.
\end{align}

Moreover, 
\begin{align}
    |N(S,v)| \leq s-r \leq s-1,\forall v \in R. 
\end{align}

This is because $p$ has the largest neighborhood in $S$ and $p$'s neighborhood is of size atmost $s-r$, and since $|S|\geq 1, s-r \leq s-1$.

Thus, Lemma 2 and Theorem 3 from ~\cite{Tomita04} hold, which implies that $T(s)=O(3^{s/3})$. Since there are $n$ vertices and their outdegree is atmost $\alpha$, the worst case running time of \scr{} (which is also an upper bound for $|sct(G)|$) is $nT(\alpha)=O(n3^{\alpha/3})$ and hence, worst case running times of \mainalg{} for obtaining global, per-vertex and per-edge clique counts are $O(n\alpha 3^{\alpha/3})$, $O(n\alpha^2 3^{\alpha/3})$ and $O(n\alpha^3 3^{\alpha/3})$, respectively.

% \begin{theorem}[Restatement of Theorem $3$ in ~\cite{tomita}]
% We have that
% \begin{align*}
%     T(s)=C3^{\frac{s}{3}}-Q(s)
% \end{align*}
% where
% \begin{align*}
% Q(s)&=q_1s^2+q_2s+q_3 \\
% q_1&=p_1/2>0, q_2=9p_1/2>0, q_3=27p_1/2>0\\
% \end{align*}
% and
% \begin{align*}
%     C=\max\{C_1, C_2, C_3\}
% \end{align*}
% where
% \begin{align*}
%     C_1&=3q_2/\ln{3}=27p_1/2\ln{3}\\
%     C_2&=39p_1/(2*3^(1/3)) \\
%     C_3&= \text{max over $s$ of } \frac{1}{3(1-2*3^{-2/3})}\frac{Q(s-3)}{3^{s/3}} 
% \end{align*}
% Note that $\frac{Q(s-3)}{3^{s/3}}$ approaches $0$ as $n \xrightarrow{}0$ and hence is bounded above. Hence, $C_3$ is well defined.
% \end{theorem}

% \begin{proof}
% Refer proof of Theorem $3$ in ~\cite{Tomita04}.
% Let $R(n)=C3^{n/3}-Q(n)$ then $R(n)$ is monotone increasing with $R(n) \geq 0 \forall n\geq 0$.

% Consider $R(x)$
\end{proof}
%%%%%%%%%%%

% Now we look at \mainalg. Note that the subsequent counting steps do \emph{not}
% need the node labels in $\bT$; for all path $T$, one only needs $P(T)$ and $H(T)$.
% The paths can be looped over by a DFS from the root. For each path,
% there are precisely $|P(T)|+1$ updates to global clique counts,
% and at most $|H(T) \cup P(T)| \times (|P(T)|+1)$ updates to per-vertex clique counts.
% The length of $T$ is at most $\alpha$, and thus both these quantities
% are $O(\alpha^2)$. Thus, the total running time is $O(\alpha^2 |\sct(G)|)=O(n\alpha^2 3^{\alpha/3})$ for global and per-vertex clique counting.

% Similarly, for each path, at most $|H(T) \cup P(T)|^2 \times (|P(T)|+1)$ updates are made to per-edge clique counts. This quantity is $O(\alpha^3)$. Thus, the total running time is $O(\alpha^3 |\sct(G)|)==O(n\alpha^3 3^{\alpha/3})$.



{\bf Storage cost:} Currently, \mainalg{} is represented through
two parts: the construction of $\sct(G)$ and then processing it to get
clique counts. Conceptually, this is cleaner to think about and it makes the proof
transparent. On the other hand, it requires storing $\sct(G)$, which is potentially
larger than the input graph. A more space efficient implementation is obtained
by combining these steps. 

We do not give full pseudocode, since it is somewhat
of a distraction. (The details can be found in the code.) Essentially,
instead of constructing $\sct(G)$ completely in breadth-first manner,
we construct it depth-first through recursion. This will loop
over all the paths of $\bT$, but only store a single path at any stage.
The updates to the clique counts are done as soon as any root to leaf
path is constructed. The total storage of a path is the storage
for all the labels on a path. As mentioned earlier in the
proof of \Thm{main}, all non-root
nodes are labeled with sets of size at most $\alpha$. The length
of the path is at most $\alpha$, so the total storage is $O(\alpha^2)$.
A classic bound on the degeneracy is $\alpha \leq \sqrt{2m}$ (Lemma 1 of~\cite{ChNi85}),
so the storage, including the input, is $O(m+n)$.

\end{proof}

% {\bf Counting upto a specific $k$:} If we are interested in counting cliques upto only a certain $k$, it is wasteful to construct the $\sct{}$ to its full depth. A naïve way to truncate the tree would be to terminate any branch that has more than $k$ edge labels of type $\mathfrak{h}$ as such a branch can never yield a unique clique of size $k$.  the number of links marked with We notice that whenever the number of vertices along any path become more than $k$, the path can never 

% Currently, \mainalg{} is represented through
% two parts: the construction of $\sct(G)$ and then processing it to get
% clique counts. Conceptually, this is cleaner to think about and it makes the proof
% transparent. On the other hand, it requires storing $\sct(G)$, which is potentially
% larger than the input graph. A more space efficient implementation is obtained
% by combining these steps. 

% In real-world graphs, degeneracy values are typically
% small (less than 100), so the extra space overhead of $O(\alpha^3)$ is minimal.

% \begin{claim} \label{clm:recur} There is an implementation of \mainalg{}
% that has the same running time, but has storage $O(m+n)$.
% \end{claim}

% \begin{proof} We do not give full pseudocode, since it is somewhat
% of a distraction. (The details can be found in the code.) Essentially,
% instead of constructing $\sct(G)$ completely in breadth-first manner,
% we construct it depth-first through recursion. This will loop
% over all the paths of $\bT$, but only store a single path at any stage.
% The updates to the clique counts are done as soon as any root to leaf
% path is constructed. The total storage of a path is the storage
% for all the labels on a path. As mentioned earlier in the
% proof of \Thm{mainalg}, all non-root
% nodes are labeled with sets of size at most $\alpha$. The length
% of the path is at most $\alpha$, so the total storage is $O(\alpha^2)$.
% A classic bound on the degeneracy is $\alpha \leq \sqrt{2m}$ (Lemma 1 of~\cite{ChNi85}),
% so the storage, including the input, is $O(m+n)$.
% \end{proof}


{\bf Parallel version of \mainalg:} While this is not central to our results,
we can easily implement a parallel version of \mainalg{} for \emph{global} clique counts.
We stress that our aim was not to delve into complicated parallel algorithms,
and merely to see if there was a way to parallelize the counting involving minimal code changes.
The idea is simple, and is an easier variant of the parallelism in kCList~\cite{DBS18}. 
Observe that the children of the root
of $\sct(G)$ correspond to finding cliques in the sets $N^+(v)$, for all $v$.
Clique counting in each of these sets can be treated as an independent problem,
and can be handled by an independent thread/subprocess. Each subprocess
maintains its own array of global clique counts. The final result
aggregates all the clique counts. The change ends up being a few lines of code
to the original implementation.

Note that this becomes tricky for local counts. Each subprocess cannot
afford (storage-wise) to store an entire copy of the local count data structure.
The aggregation step would be more challenging. Nonetheless, it should be feasible
for each subprocess to create local counts for $N^+(v)$, and appropriately
aggregate all counts. We leave this for future work.
% We also implement a node-parallel version of this algorithm by running the ``for'' loop of \Step{for-parallel} in parallel for each $v \in V$. We only implement for counting $k-$cliques and not for per-vertex and per-edge $k-$cliques. The update of the result data structures $T_k, T_V, T_E$ cannot happen in parallel and to deal with this, we use the inbuilt primitives which essentially create a copy of these data structures, one copy for each thread. Since these structures can become very large when obtaining per-vertex and per-edge counts, we skip parallelization for them. Note that this is a solvable problem since at any time, a given thread is dealing with a subgraph of size atmost $\alpha$ and hence, instead of replicating the entire resultant data structure, we can simply create a smaller data structure for each thread and combine the results once all the threads have finished executing. However, this optimization is out of the scope of this paper. 

{\bf Counting $k$-cliques for a specific $k$:} \mainalg{} can be modified to obtain clique counts upto a certain user specified $k$ (instead of counting for all $k$). Whenever the number of links marked $\mathfrak{h}$ becomes greater than $k$ in any branch of the computation, we simply truncate the branch (as further calls in the branch will only yield cliques of larger sizes). 


%%%%%%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse

\subsection{Preliminaries} \label{sec:prelim}
We consider the graph to be undirected. Let $G(V, E)$ denote the input graph and let $n=|V|, m=|E|$. Let $\alpha$ denote the degeneracy of the graph. Let $C$ denote the total number of cliques in $G$, $C_k$ denote the number of $k-$cliques in $G$, $C_k^v$ denote the number of $k-$cliques that vertex $v$ is a part of and let $C_k^{(u,v)}$ where $u<v$ denote the number of $k-$cliques that edge $(u,v)$ is a part of.

\subsection{Main algorithm} \label{sec:main}

% We first describe the basic framework of our algorithm and show that the recursion tree has size $O(n3^{\alpha/3})$. 

The basic framework of our algorithm follows that of \Eppstein{} very closely. Similar to \Eppstein{}, at the first level, the algorithm simply constructs a DAG using the degeneracy ordering. For every $v \in V$, it sets $H = \{v\}, D=\emptyset$ and passes $D, H$ and the appropriate $P$ to the recursive routine \mainalgrec{} which is a modified version of \BK{}. The pivot is chosen from $P$ in \Step{pivot}. When $P$ is empty, the appropriate clique counts are updated and the function returns. Depending on whether we want $k-$clique counts, per-vertex $k-$clique counts or per-edge $k-$clique counts, we call $func-k, func-V, func-E$ resp. Thus, line starting with $\#$ is called to calculate per-vertex counts and line starting with $\$$ is called to calculate per-edge counts.

% \begin{algorithm}
% \caption{\mainalgrecAlt($H, D, P$) \newline
% Input: \newline
% $H$: vertices that are necessarily a part of the clique \newline 
% $D$: vertices that can be dropped from the clique \newline 
% $P$: vertices that can be used to extend the clique 
% }
% If $P==\emptyset$:\\
% \ \ \ \ $T = T + 2^{|D|}$ \\
% \ \ \ \ $func(H,D)$ \\ \label{step:func}
% \ \ \ \ return \\
% Let $N_v$ denote the neighborhood of $v$ in $G$. \\
% Choose a pivot $u \in P$ that maximizes $P \cap N_u$ \\ \label{step:pivot}
% For each $v \in P \setminus N_u$: \\
% \ \ \ \ if $v == u$: $\mainalgrecAlt{(H, D \cup \{u\}, P \cap N_u)}$ \\ \label{step:pivot-call}
% \ \ \ \ else $\mainalgrecAlt{(H \cup \{v\}, D, P \cap N_v)}$ \\ \label{step:non-pivot-call}
% \ \ \ \ $P \leftarrow P \setminus \{v\}$ 
% \end{algorithm}

\begin{algorithm}
\caption{\mainalgrec($H, D, P$) \newline
Input: \newline
$H$: vertices that are necessarily a part of the clique \newline 
$D$: vertices that can be dropped from the clique \newline 
$P$: vertices that can be used to extend the clique 
}
If $P==\emptyset$:\\ \label{step:P}
% \ \ \ \ $T = T + 2^{|D|}$ \\
% \ \ \ \ $func-k(H,D)$ \\ \label{step:func-k}
\ \ \ \ for $i=0$ to $|D|$: \\ \label{step:count-k}
\ \ \ \ \ \ \ \ Increment $T_k[|H|+|D|-i]$ by ${|D| \choose i}$ \\
\ \ \ \ \#$func-V(H,D)$ \\ \label{step:func-V}
\ \ \ \ \$$func-E(H,D)$ \\ \label{step:func-E}
\ \ \ \ return \\
% Let $N_v$ for $v \in V$ denote the neighborhood of $v$ in $P$. \\
Choose a pivot $u \in P$ that maximizes number of neighbors of $u$ in $P$\\ \label{step:pivot}
Let $N=\{v | (u,v) \in E, v \in P\}$ denote the neighbors of $u$ in $P$ \\ \label{step:N}
Let $W=P \setminus N \setminus \{u\}$ denote the set of non-neighbors of $u$ in $P$ \\ \label{step:W}
Form an ordering $\Phi$ of the vertices in $P$ that is of the form $w_1, w_2,...,u,v_1, v_2,...$ where $w_i \in W$ and $v_i \in N$ \\ \label{step:Phi}
Convert $G_{|P}$ into DAG using $\Phi$ and let $N_v^+$ denote the outneighborhood of $v$ in the DAG. \\
$\mainalgrec{(H, D \cup \{u\}, N)}$ \\ \label{step:pivot-call}
For $w \in W$:\\
\ \ \ \ $\mainalgrec{(H \cup \{w\}, D, N_w^+)}$ \\ \label{step:non-pivot-call}
\end{algorithm}

\begin{claim} \label{clm:HDP}
Consider any call to \mainalgrec{}. The following invariants hold: Let $R=H \cup D$. Then $R$ is a clique. $H$, $D$ and $P$ are disjoint and $P$ is a set of vertices connected to all vertices in $R$.
\end{claim}
\begin{proof} 
We will prove by induction.
Initially, $D$ is empty, $H=\{v\}$ and $P=N_v^+$ according to the degeneracy ordering. Thus, the conditions are trivially true.

Suppose the conditions hold for some intermediate call of \mainalgrec{}. For subsequent calls made in \Step{non-pivot-call}, for any $w \in W$, $H \cup \{w\} \cup D$ is a clique and  $N_w^+$ (according to $\Phi$) is a set of vertices connected to every vertex in the clique. Thus, all the conditions are true. Same is true for call made in \Step{pivot-call}. 
\end{proof}

% \begin{claim}

% \end{claim}
% \begin{proof}
% \end{proof}

\begin{claim} \label{clm:ordering-unique}
Given a set $P$ of vertices, an ordering of the vertices in $P$, and any clique $C \subseteq P $ there is exactly one $v$ such that $C$ can be written as $\{v\} \cup B$ for some $B \subseteq N_v^+$, where $N_v^+$ is the outneighborhood of $v$ when $P$ is converted into a DAG according to the given ordering.
\end{claim}
\begin{proof}
For the given clique $K$, let $v$ be the lowest vertex in the clique according to the given ordering. Let $B=K \setminus \{v\}$ then $B \subseteq N_v^+$. Thus, $v$ exists. For any other vertex $v' \in K$, $v$ would not be in $N_{v'}^+$. Thus $v$ is unique. Hence, proved.
\end{proof}

\begin{lemma} \label{lem:K}
Let $C(P)$ denote the set of cliques in $P$. Let $\K(H,D,P)$ represent the set of all cliques of the form $H \cup \Delta \cup C$ where $\Delta \subseteq D$ and $C \in C(P)$. 

Let $u$ be the pivot chosen in \Step{pivot}, $N=N_u^+$ represent the (out)neighborhood of $u$, $W = P \setminus N \setminus \{u\}$ represent the set of non-neighbors of $u$ (as set in the algorithm). Let the vertices be ordered according to $\Phi$ as described in \Step{Phi}. Let $\K_u = \K(H, D \cup \{u\}, N)$ and let, $\forall w \in W, \K_w = \K(H \cup \{w\}, D, N_w^+)$. 

Then for every clique $K \in \K(H,D,P)$, either $K \in \K_u$ and $K \notin \K_w$ for all $w \in W$, or $K \in K_w$ for exactly one $w \in W$ and $K \notin K_u$. 
\end{lemma}
\begin{proof}
Exactly one of the following has to be true for $K$: 
\begin{enumerate} 
\item $K$ contains a non-neighbor $v$ of $u$. Let $C = K \setminus H \setminus D$ be the part obtained from $P$. Then, by \Clm{ordering-unique} and the choice of $\Phi$ such that all non-neighbors occur before $u$ and neighbors of $u$ in the ordering, there $\exists$ unique $w \in W$ such that $B \subseteq N_w^+$ i.e. $K \in \K_w$. Moreover, since $K$ contains a non-neighbor of $u$, $K \notin \K_u$.
\item $K$ contains $u$. Then $\forall w \in W$, $K \notin \K_w$ and $K  \setminus H \setminus D \subseteq N$ i.e. $K \in \K(H, D \cup \{u\}, N)$ i.e. $K \in \K_u$.
\item $K$ contains only neighbors of $u$ but not $u$, then $\forall w \in W$, $K \notin \K_w$. Moreover, $K  \setminus H \setminus D \setminus \{u\} \subseteq N$. Hence, $K \in \K(H, D \cup \{u\}, N)$ i.e. $K \in \K_u$.

\end{enumerate}
Thus, the conditions are true in all cases. Hence, proved. Thus, $\K(H,D,P)=\bigcup_{w \in W}\K_w \cup \K_u$ and $|\K(H,D,P)|=|\bigcup_{w \in W}\K_w \cup \K_u|$.
\end{proof}

\begin{theorem}
When \mainalg{} returns, $T[k]=|C_k|$.
 % Moreover, 
\end{theorem}

\begin{proof}
Let $C$ be the set of all cliques in $G$. By \Clm{ordering-unique}, $C=\bigcup\limits_{v \in V} (\{v\} \cup \{ C(N_v^+)\}=\bigcup\limits_{v \in V} \K(\{v\}, \emptyset, N_v^+)$.  

Let $ \bf{S}$ be the set of all $(H, D, \emptyset)$ obtained by \mainalg{} (i.e. when $P$ is empty). By \Lem{K}, and abusing notation slightly, $\bigcup\limits_{S \in \bf{S}}\K(S) = C$ and $|C_k|=\sum\limits_{(H, D, \emptyset) \in \bf{S}}{|D| \choose k-|H|}=T[k]$. 
\end{proof}

Let $T(n)$ be the worst case running time of \mainalgrec{} when $|P|=n$.

Let $Q=P \setminus N_u$. Let $T_q(n)$ be the worst case running time of \mainalgrec{} when $|P|=n$ and $|Q|=q$. Note that when $P$ is passed to \mainalgrec{}, it calls \mainalgrec{} a total of $q$ times. 

Thus, $T(n)=\max\limits_q\{T_q(n)\}$. 

Note that all steps other than \Step{pivot-call} and \Step{nonpivot-call} take time $O(n^2)$. Say, they take time $p_1n^2$, where $p_1>0$ is a constant.

Thus, we have that:
\begin{align}
    T_q(n) \leq \sum\limits_{v \in Q}{T(|N_v^+|) 
    + p_1n^2}.
\end{align}

Moreover, 
\begin{align}
    |N_v^+| \leq n-q \leq n-1,\forall v \in Q. 
\end{align}

This is because $u$ has the largest neighborhood in $P$ and $u$'s neighborhood is of size atmost $n-q$, and since $|P|\geq 1, n-q \leq n-1$.

\begin{theorem}[Restatement of Theorem $3$ in ~\cite{tomita}]
We have that
\begin{align*}
    T(n)=C3^{\frac{n}{3}}-Q(n)
\end{align*}
where
\begin{align*}
Q(n)&=q_1n^2+q_2n+q_3 \\
q_1&=p_1/2>0, q_2=9p_1/2>0, q_3=27p_1/2>0\\
\end{align*}
and
\begin{align*}
    C=\max\{C_1, C_2, C_3\}
\end{align*}
where
\begin{align*}
    C_1&=3q_2/\ln{3}=27p_1/2\ln{3}\\
    C_2&=39p_1/(2*3^(1/3)) \\
    C_3&= \text{max over $n$ of } \frac{1}{3(1-2*3^{-2/3})}\frac{Q(n-3)}{3^{n/3}} 
\end{align*}
Note that $\frac{Q(n-3)}{3^{n/3}}$ approaches $0$ as $n \xrightarrow{}0$ and hence is bounded above. Hence, $C_3$ is well defined.
\end{theorem}

\begin{proof}
Refer proof of Theorem $3$ in ~\cite{Tomita04}.
% Let $R(n)=C3^{n/3}-Q(n)$ then $R(n)$ is monotone increasing with $R(n) \geq 0 \forall n\geq 0$.

% Consider $R(x)$
\end{proof}

\begin{corollary}
The running time of \mainalg{} is $O(n\alpha3^{\alpha/3})$ for counting $k-$cliques.
\end{corollary}
\begin{proof}
\Step{count-k} is executed only for the leaves and since the maximum size of any outneighborhood and any clique = $\alpha$, this completes the proof.
\end{proof}

 
% \Shweta{\subsection{Main algorithm - old proof}
% Let $G(V,E)$ be the input graph. We consider the graph to be undirected. Let $C_k(P)$ denote the set of $k-$cliques in $G_{|P}$. Let $\rho(P)$ represent the edge density of $G_{|P}$. We will say $u$ is a neighbor of $v$ if $(u,v) \in E$ and non-neighbor otherwise, and vice versa. Let, for set $S$ of cliques, $S_k = \{K| K \in S, |K|=k\}$ denote the set of $k$-cliques in $S$. 

% % \begin{algorithm}
% % \caption{\cliquecounter($P$) \newline
% % Input: \newline
% % $P$: set of vertices from the input graph that we want to count all cliques in. \newline 
% % Output: \newline
% % Array $C[k]$ where $C[k] = |C^k(P)|, \forall k \in [0,|P|]$ 
% % }
% % Let $C$ be an array of size $|P|+1$ initialized to 0. \label{initialize}\\
% % % if $|P|==0:$ \\
% % % \ \ \ \ $\hc[0] = 1,$ return $\hc$ \\ 
% % % if $|P|==1:$ \\
% % % \ \ \ \ $\hc[0] = 1, \hc[1] = 1,$ return $\hc$ \\ 
% % if $|P| \leq 1$ or $\rho(P) == 1$: \label{condition-base}\\
% % \ \ \ \ for $k=0$ to $|P|$: \label{loop-base}\\
% % \ \ \ \ \ \ \ \ $C[k] = {|P| \choose k}$ \label{value-base}\\
% % \ \ \ \ return $C$ \label{base} \\ 
% % Let $u$ be the vertex in $P$ that maximizes $P \cap \Gamma(u)$ \label{step:defu}\\ 
% % For $v \in P \setminus \Gamma(u)$: \\
% % \ \ \ \ Let $P_v = P \cap \Gamma(v)$ \\
% % \ \ \ \ $C_v = \cliquecounter(P_v)$ \label{Cv} \\
% % \ \ \ \ for $k=1$ to $|P_v|$: \\
% % \ \ \ \ \ \ \ \ $C[k] = C[k] + C_v[k-1]$ \\
% % \ \ \ \ \ \ \ \ if $v == u$: \\
% % \ \ \ \ \ \ \ \ \ \ \ \ $C[k] = C[k] + C_v[k]$ \\
% % \ \ \ \ $P = P \setminus \{v\}$ \\
% % $C[0] = 1$ \\
% % return $C$
% % % \ \ \ \ $C[]
% % % $\hc = $ \\
% % % if $R \cup P = \emptyset$ then \\
% % % \ \ \ \ report $R$ as a maximal clique \\
% % % end if \\
% % % for each $v \in P$ do \\
% % % \ \ \ \ \bronkerbosch$(P \cap \Gamma(v), R \cup \{v\}, X \cap \Gamma(v))$ \\
% % % \ \ \ \ $P \leftarrow P \setminus \{v\} $ \\
% % % \ \ \ \ $X \leftarrow X \cup \{v\} $ \\
% % \end{algorithm}

% \begin{algorithm}
% \caption{\mainalg($P$) \newline
% Input: \newline
% $P$: set of vertices from the input graph that we want to count all cliques in. \newline 
% Output: \newline
% Array $C[k]$ where $C[k] = |C_k(P)|, \forall k \in [0,|P|]$ 
% % and $C[k]=0$ for all other $k$. 
% }
% Let $C$ be an array of size $|P|+1$ initialized to 0. \label{step:initialize}\\
% % if $|P|==0:$ \\
% % \ \ \ \ $\hc[0] = 1,$ return $\hc$ \\ 
% % if $|P|==1:$ \\
% % \ \ \ \ $\hc[0] = 1, \hc[1] = 1,$ return $\hc$ \\ 
% if $|P| \leq 1$ or $\rho(P) == 1$: \label{step:condition-base}\\
% \ \ \ \ For $k=0$ to $|P|$: \label{step:loop-base}\\
% \ \ \ \ \ \ \ \ $C[k] = {|P| \choose k}$ \label{step:value-base}\\
% \ \ \ \ return $C$ \label{step:base} \\ 
% Let $u$ be the vertex in $P$ that maximizes $P \cap \Gamma(u)$ \label{step:defu}\\
% % Let $N=\{v|v \in P, $v \noteq u, (v,u) \notin G_{|P}\}$.
% Let $N=P \cap \Gamma(u)$ represent the neighbors of $u$ in $P$. \\
% Let $\bar{N}= P \setminus N \setminus \{u\}$ be the set of non-neighbors of $u$ excluding $u$\\
% Let, for set of vertices $S$, $\Phi(S)$ denote the ordering of vertices in $S$ in increasing order of their id  \\
% Let $\Phi(S) \cdot \Phi(T)$ represent the concatenation of increasing order of vertices in $S$ and increasing order of vertices in $T$.\\
% Consider the ordering $\Phi(\bar{N}) \cdot u \cdot \Phi{N}$ and form a DAG $DG$ by using this ordering on $P$.\\
% For $v\in P,$ let $N^+_v$ represent the outneighborhood of $v$ in $DG$ \\
% Let $C_N = \mainalg{}(N_u^+)$ \label{step:CN} \\
% For $k=1$ to $|N_u^+|$: \\
% \ \ \ \ $C[k] = C_N[k] + C_N[k-1]$ \label{step:C-k}\\
% $C[|N_u^+|+1] = C_N[|N_u^+|]$ \label{step:N+1}\\
% For $v \in \bar{N}$: \label{step:loop-bar-N}\\
% % \ \ \ \ Let $P_v = P \cap \Gamma(v)$ \\
% \ \ \ \ $C_v = \mainalg{}(N_v^+)$ \label{step:Cv} \\
% \ \ \ \ for $k=1$ to $|N_v^+|$: \\
% \ \ \ \ \ \ \ \ $C[k] = C[k] + C_v[k-1]$ \label{step:C-bar-N}\\
% % \ \ \ \ \ \ \ \ if $v == u$: \\
% % \ \ \ \ \ \ \ \ \ \ \ \ $C[k] = C[k] + C_v[k]$ \\
% % \ \ \ \ $P = P \setminus \{v\}$ \\
% $C[0] = 1$ \label{step:C-0}\\
% return $C$
% % \ \ \ \ $C[]
% % $\hc = $ \\
% % if $R \cup P = \emptyset$ then \\
% % \ \ \ \ report $R$ as a maximal clique \\
% % end if \\
% % for each $v \in P$ do \\
% % \ \ \ \ \bronkerbosch$(P \cap \Gamma(v), R \cup \{v\}, X \cap \Gamma(v))$ \\
% % \ \ \ \ $P \leftarrow P \setminus \{v\} $ \\
% % \ \ \ \ $X \leftarrow X \cup \{v\} $ \\
% \end{algorithm}


% % \begin{claim}
% % Let $|P|>=1$ and let $u$ be as defined in \Step{defu}. Let $C(P)$ denote the set of all cliques in $G_{|P}$ and let
% % \begin{itemize}
% %     \item $C_u$ be the set of cliques in $G_{|P}$ that contain $u$
% %     \item $C_n$ be the set of cliques in $G_{|P}$ that contain only neighbors of $u$ (and hence, does not contain $u$
% %     \item $C_{\bar{N}}$ be the set of cliques in $G_{|P}$ that contain a non-neighbor of $u$ other than $u$
% % \end{itemize}

% % Then $C(P) = C_u \cup C_n \cup C_{\bar{N}}$ and $C_u, C_n, C_{\bar{N}}$ are mutually disjoint.
% % \end{claim}
% % \begin{proof}
% % Let $K$ be a clique in $G_{|P}$. Then $K$ either contains $u$ or does not contain $u$ - but both ca\bar{N}ot be true simultaneously. 

% % If $u \in K$, by definition, $K \in C_u$. Since $u$ is not a neighbor of $u$, $K \notin C_n$. Moreover, if $\bar{N}br \in P$ is a non-neighbor of $u$ i.e. $(u,\bar{N}br) \notin E(G_{|P})$ then $u$ and $\bar{N}br$ ca\bar{N}ot both be in $K$. Thus, $K \notin C_{\bar{N}}$. The other cases can be proved similarly. 
% % \end{proof}

% % \begin{claim}
% % Let $|P|>1$ and let $u$ be as defined in \Step{defu}. Let $C(P)$ denote the set of all cliques in $G_{|P}$ and let
% % \begin{itemize}
% %     \item $C_u$ be the set of cliques in $G_{|P}$ that contain $u$
% %     \item $C_n$ be the set of cliques in $G_{|P}$ that contain only neighbors of $u$ (and hence, does not contain $u$
% %     \item $C_{\bar{N}}$ be the set of cliques in $G_{|P}$ that contain a non-neighbor of $u$ other than $u$
% % \end{itemize}

% % Then every clique in $P$ belongs to exactly one of $C_u, C_n, C_{\bar{N}}$.
% % \end{claim}
% % \begin{proof}
% % Let $K$ be a clique in $G_{|P}$. Then $K$ either contains $u$ or does not contain $u$ - but both ca\bar{N}ot be true simultaneously. 

% % If $u \in K$, by definition, $K \in C_u$ and $K \notin C_n$. Moreover, for any clique $J \in C_{\bar{N}}$, $J$ contains a non-neighbor of $u$ i.e. $\exists \bar{N}br \in J$ such that $(u,\bar{N}br) \notin E(G_{|P})$ but this violates the definition of a clique thus $J$ ca\bar{N}ot be a clique, which is a contradiction. 

% % If $u \notin K$, then $K$ either contains a non-neighbor of $u$, in which case, by definition, $K \in C_{\bar{N}}$ and $K \notin C_n$, or $K$ does not contain any non-neighbor of $u$, in which case, by definition, $K \notin C_{\bar{N}}$ and $K \in C_n$. Hence, proved.
% % \end{proof}

% \begin{claim}
% Let $|P|>=1$ and let $u$ be as defined in \Step{defu}. Let $C_k(P)$ denote the set of all \kcs{} in $G_{|P}$ for $k>=0$ and let
% \begin{itemize}
%     \item $C_k(uN)$ be the set of \kcs{} in $G_{|P}$ that \textbf{contain} $u$
%     \item $C_k(N)$ be the set of \kcs{} in $G_{|P}$ that contain only neighbors of $u$ (and hence, do not contain $u$)
%     \item $C_k(\bar{N}N)$ be the set of \kcs{} in $G_{|P}$ that contain a non-neighbor of $u$ 
%     % other than $u$
% \end{itemize}

% Then every \kc{} in $P$ belongs to exactly one of $C_k(uN), C_k(N), C_k(\bar{N}N)$.
% \end{claim}
% \begin{proof}
% Let $K$ be a \kc{} in $G_{|P}$. Then $K$ either contains $u$ or does not contain $u$ - but both cannot be true simultaneously. 

% If $u \in K$, by definition, $K \in C_k(uN)$ and $K \notin C_k(N)$. Suppose $K \in C_k(\bar{N}N)$, then $K$ contains a non-neighbor of $u$ i.e. $\exists nn \in K$ such that $(u,nn) \notin E(G_{|P})$ but this violates the definition of a clique so $K$ must not be a clique, which is a contradiction. 

% If $u \notin K$, then $K$ either contains a non-neighbor of $u$, in which case, by definition, $K \in C_k(\bar{N}N)$ and $K \notin C_k(N)$, or $K$ does not contain any non-neighbor of $u$, in which case, by definition, $K \notin C_k(\bar{N}N)$ and $K \in C_k(N)$. Hence, proved.
% \end{proof}

% \begin{corollary} \label{cor:eq}
% $C_k(uN), C_k(N)$ and $C_k(\bar{N}N)$ are disjoint and $C_k(P)= C_k(uN) \cup C_k(N) \cup C_k(\bar{N}N)$, which implies $|C_k(P)| = |C_k(uN)| + |C_k(N)| + |C_k(\bar{N}N)|$.
% \end{corollary}


% \begin{claim} \label{clm:same}
% $C_k(uN) = \{\{u\} \cup K | K \in C_{k-1}(N)\}$ and $|C_k(uN)|=|C_{k-1}(N)|$.
% \end{claim}
% \begin{proof}
% Let $S=\{\{u\} \cup K | K \in C_{k-1}(N)\}$.
% Let $J\in C_k(uN)$. Let $Q = J \setminus \{u\}$ then $Q$ is a $(k-1)$-clique comprising of only neighbors of $u$ i.e. $Q \in C_{k-1}(N)$. Thus, $Q \cup \{u\}  \in S$ . Thus, $J \in S$.

% Now, consider some $J \in S$. Then $J=\{u\} \cup K$ for some $K \in C_{k-1}(N)$. But $K$ is a clique comprising  of only neighbors of $u$. Thus, $K \cup \{u\}$ is also a clique and it contains $u$, hence $J \in C_{k}(uN)$. 

% Moreover, since $\forall K \in C_{k-1}(N)$ we have that $u \notin K$ therefore, $K \cup \{u\}$ is a unique \kc{} in $G$, which implies that $|\{\{u\} \cup K | K \in C_{k-1}(N)\}| = |C_{k-1}(N)|$ i.e.  $|S|=|C_{k-1}(N)|$ i.e. $|C_k(uN)|=|C_{k-1}(N)|$. Hence, proved.
% \end{proof}

% \begin{claim}\label{clm:CkP}
% $|C_k(P)| = |C_k(\bar{N}N)| + |C_{k-1}(N)| + |C_k(N)|$.
% \end{claim} 
% \begin{proof}
% Substituting from \Clm{same} in \Cor{eq}.
% \end{proof}

% % \begin{theorem}
% % When \cliquecounter{} returns, $C[k]=C^k(P)$ for $0 \leq k \leq |P|$.
% % \end{theorem}
% % \begin{proof}
% % We will prove this using induction on $|P|+k$.
% % Suppose the claim is true for some $N=|P|+k$. We want to prove that the claim is true also for $N+1$. 

% % For the base case, when $N=0, |P|=0, k=0,$ the loop in \Step{loop-base} is evaluated for $i=0$ and \Step{base} returns $C[0]=1$. Hence, the claim is true. For $N=1$, if $|P|=0$ and $k=1$, loop runs only for $i=0$, thus $C[1]$ is left unchanged and \Step {base} returns $C[1]=0$. Thus, the claim is true in this case.

% % For $N=1$, if $|P|=1$ and $k=0$, \Step{loop-base} sets $C[0]=1$ and returns in \Step{base}. Thus, the claim is true in this case as well.

% % Suppose the claim is true for all $N \leq N'$ i.e. Consider some $|P|$ and $k$ such that $|P|+k=N+1$. 

% % \end{proof}

% \begin{claim}
% $N=N_u^+$. \label{clm:N}
% \end{claim}
% \begin{proof}
% Since all the neighbors of $u$ in $P$ are after $u$ in the ordering, if for $v \in P, (u,v) \in E(G)$ then $v \in N_u^+$ i.e. $N=N_u^+$.
% \end{proof}

% \begin{claim}
% $C_k(\bar{N}N)=\bigcup\limits_{v \in \bar{N}}\bigcup\limits_{J \in C_{k-1}(N_v^+)}\{\{v\} \cup J\}$ and $|C_k(\bar{N}N)|=\sum\limits_{v \in \bar{N}}|C_{k-1}(N_v^+)|$.
% \end{claim}

% \begin{proof}
% If we ascribe a clique $K$ in $C_k(\bar{N}N)$ to the lowest  non-neighbor in $K$ according to the ordering, then this induces a partition over $C_k(\bar{N}N)$.

% % Let $\pi(v)$ for $v \in P$ denote the 
% Let, for $v \in \bar{N}$, $C_k^{v}=\{K|K \in C_k(P), v \in K$ and $v$ is the lowest vertex in $K$ according to the ordering$\}$. Then, $C_k(\bar{N}N)=\bigcup\limits_{v \in \bar{N}}C_k^{v}$ and $|C_k(\bar{N}N)|=\sum\limits_{v \in \bar{N}}|C_k^{v}|$.

% We will show that $\bigcup\limits_{J \in C_{k-1}(N_v^+)}\{\{v\} \cup J\}=C_k^v$.

% Let for $ v \in P, \pi(v)$ give the position of $v$ in the ordering.

% For any $v \in \bar{N}$, for any $K \in C_k^v$, for any $w \in K, w \neq v$ we have that $ \pi(w)>\pi(v)$ and $(v,w) \in E(G)$ so $w \in N^+_v$ and this is true for all vertices in $K\setminus \{v\}$ i.e. $K \setminus \{v\} \subseteq N^+_v$ i.e. $K \setminus \{v\} \in C_{k-1}(N_v^+)$ i.e. $K \in \bigcup\limits_{J \in C_{k-1}(N_v^+)}\{\{v\} \cup J\}$.

% For $J \in C_{k-1}(N_v^+)$, $\{v\} \cup J$ is a \kc{} with $v$ as the lowest vertex according to the ordering. Hence, $\{v\} \cup J \in C_k^v$. 

% Moreover, since $v \notin J$, $\{v\} \cup J$ is a unique \kc{} in $P$. Hence, $|C_k^v|=|C_{k-1}(N_v^+)|$ i.e. $|C_k(\bar{N}N)|=\sum\limits_{v \in \bar{N}}|C_{k-1}(N_v^+)|$.

% Hence, proved.

% \end{proof}

% \begin{theorem}
% When \mainalg{} returns, $C[k]=|C_k(P)|$ for $0 \leq k \leq |P|$.
% \end{theorem}
% \begin{proof}
% We will prove this using induction on the size of $P$. 
% For the base case, when $ p=|P|=0$ the loop in \Step{loop-base} is evaluated for $k=0$ and \Step{base} returns $C[0]=1$. $C[1]$ is still $0$. Hence, the claim is true. 

% % For $N=1$, if $|P|=0$ and $k=1$, loop runs only for $i=0$, thus $C[1]$ is left unchanged and \Step {base} returns $C[1]=0$. Thus, the claim is true in this case.

% For $p=1$, 
% % if $|P|=1$ and $k=0$,
% \Step{loop-base} sets $C[0]=1, C[1]=1$ and returns in \Step{base}. Thus, the claim is true in this case as well. 

% Suppose the claim if true for $|P|=p'$, i.e. when $|P| \leq p'$, \mainalg{} returns $C$ such that $C[k]=|C_k(P)|$ for $0 \leq k \leq p'$.
% We will prove that the claim holds true even when $|P|=p'+1$.

% If $P$ is a clique i.e. $\rho_2(P) == 1$, then for $0 \leq k \leq p'+1$, $C[k]$ is set to ${|P| \choose k}$ for all $0 \leq k \leq p'+1$ and returned in \Step{base}. Thus the claim is true in this case.

% If $\rho_2(P) < 1$, since $|P|>1$, $\exists u$ as defined in \Step{defu}.

% $|N_u^+| \leq p'$. Thus, by the induction hypothesis, \mainalg{}($N_u^+$) returns $C_N$ such that $C_N[k]=|C_k(N_u^+)|=|C_k(N)|$ by \Clm{N}, for all $0 \leq k \leq |N_u^+|$.

% In \Step{C-k}, $C[k]$ is set to $|C_k(N)|+|C_{k-1}(N)|$. In \Step{N+1}, $C[|N|+1]$ is set to $C_N[|N|]+0=|C_{|N|}(N)|+|C_{|N|+1}(N)|$.

% The for loop of \Step{loop-bar-N} $\forall v \in \bar{N}$, calls \mainalg{($N_v^+$)}. $|N_v^+| \leq p'$ and hence $C_v$ returned by \mainalg{} is such that $C_v[k]=|C_k(N_v^+)|$. Thus, \Step{C-bar-N} adds $|C_{k}(\bar{N}N)|$ to $C[k]$.

% Thus, when the function returns, $C[k]=|C_k(N)|+|C_{k-1}(N)|+|C_k(\bar{N}N)|=|C_k(P)|$ by \Clm{CkP}. Hence, proved.
% \end{proof}

% % \begin{theorem}
% % The worst case time complexity of \cliquecounter{} is blah.
% % \end{theorem} 

% % \begin{proof}
% \subsection{Running time}
% The following is almost identical to the proofs of Lemma $2$ and Theorem $3$ in ~\cite{tomita}.

% Let $T(n)$ be the worst case running time of \mainalg{} when $|P|=n$.

% Let $R=P \setminus N = \bar{N} \cup \{u\}$. Let $T_r(n)$ be the worst case running time of \mainalg{} when $|P|=n$ and $|R|=r$. Note that \mainalg{$(P)$} calls \mainalg{} a total of $r$ times. 

% Thus, $T(n)=\max\limits_r\{T_r(n)\}$. 

% Note that all steps other than \Step{CN} and \Step{Cv} take time $O(n^2)$. Say, they take time $p_1n^2$, where $p_1>0$ is a constant.

% Thus, we have that:
% \begin{align}
%     T_r(n) \leq \sum\limits_{v \in R}{T(|N_v^+|) 
%     + p_1n^2}.
% \end{align}

% Moreover, 
% \begin{align}
%     |N_v^+| \leq n-r \leq n-1,\forall v \in R. 
% \end{align}

% This is because $u$ has the largest neighborhood in $P$ and $u$'s neighborhood is of size atmost $n-r$, and since $|P|\geq 1, n-r \leq n-1$.

% % We will prove by induction that
% \begin{theorem}[Restatement of Theorem $3$ in ~\cite{tomita}]
% We have that
% \begin{align*}
%     T(n)=C3^{\frac{n}{3}}-Q(n)
% \end{align*}
% where
% \begin{align*}
% Q(n)&=q_1n^2+q_2n+q_3 \\
% q_1&=p_1/2>0, q_2=9p_1/2>0, q_3=27p_1/2>0\\
% \end{align*}
% and
% \begin{align*}
%     C=\max\{C_1, C_2, C_3\}
% \end{align*}
% where
% \begin{align*}
%     C_1&=3q_2/\ln{3}=27p_1/2\ln{3}\\
%     C_2&=39p_1/(2*3^(1/3)) \\
%     C_3&= \text{max over $n$ of } \frac{1}{3(1-2*3^{-2/3})}\frac{Q(n-3)}{3^{n/3}} 
% \end{align*}
% Note that $\frac{Q(n-3)}{3^{n/3}}$ approaches $0$ as $n \xrightarrow{}0$ and hence is bounded above. Hence, $C_3$ is well defined.
% \end{theorem}

% \begin{proof}
% Refer proof of Theorem $3$ in ~\cite{tomita}.
% % Let $R(n)=C3^{n/3}-Q(n)$ then $R(n)$ is monotone increasing with $R(n) \geq 0 \forall n\geq 0$.

% % Consider $R(x)$
% \end{proof}

% \begin{corollary}
% There exists an algorithm, \mainalg{}{}, that counts all cliques in a graph on $n$ vertices in time $O(3^{n/3})$.
% \end{corollary}
% }

\subsection{Counting cliques per vertex} \label{sec:cliques-V}

\begin{algorithm}
\caption{\funcV ($H, D$) \newline
Input: \newline
$H$: vertices that are necessarily a part of the clique \newline 
$D$: vertices that can be dropped from the clique \newline 
}
for $v \in H$:\\
\ \ \ \ for $i=0$ to $|D|$: \\
\ \ \ \ \ \ \ \ Increment $T_V[v, |H|+|D|-i]$ by ${|D| \choose i}$ \\
for $v \in D$:\\
\ \ \ \ for $i=0$ to $|D|-1$: \\
\ \ \ \ \ \ \ \ Increment $T_V[v, |H|+|D|-i]$ by ${|D|-1 \choose i}$ \\
\end{algorithm}

\begin{lemma}
Let $T_f=$ time taken by \funcV{}. Then, $T_f=O(\alpha^2)$.
\end{lemma}
\begin{proof}
Note that $H \cup D$ is a clique. Since the largest clique can be of size atmost $\alpha$, this completes the proof.
\end{proof}
\subsection{Counting cliques per edge} \label{sec:cliques-E}

\begin{algorithm}
\caption{\funcE ($H, D$) \newline
Input: \newline
$H$: vertices that are necessarily a part of the clique \newline 
$D$: vertices that can be dropped from the clique \newline 
}
for $u \in H$:\\
\ \ \ \ for $v \in H, v>u$:\\
\ \ \ \ \ \ \ \ for $i=0$ to $|D|$: \\
\ \ \ \ \ \ \ \ \ \ \ \ Increment $T_E[u, v, |H|+|D|-i]$ by ${|D| \choose i}$ \\
for $u \in H$:\\
\ \ \ \ for $v \in D, v>u$:\\
\ \ \ \ \ \ \ \ for $i=0$ to $|D|-1$: \\
\ \ \ \ \ \ \ \ \ \ \ \ Increment $T_E[u, v, |H|+|D|-i]$ by ${|D|-1 \choose i}$ \\
for $u \in D$:\\
\ \ \ \ for $v \in D, v>u$:\\
\ \ \ \ \ \ \ \ for $i=0$ to $|D|-2$: \\
\ \ \ \ \ \ \ \ \ \ \ \ Increment $T_E[u, v, |H|+|D|-i]$ by ${|D|-2 \choose i}$ \\
\end{algorithm}

\begin{lemma}
Let $T_f=$ time taken by \funcE{}. Then, $T_f=O(\alpha^3)$.
\end{lemma}
\begin{proof}
Note that $H \cup D$ is a clique. Since the largest clique can be of size atmost $\alpha$, this completes the proof.
\end{proof}

\begin{lemma}
\end{lemma}
\fi
%%%%%%%%%%%%%%%%%% END OLD %%%%%%%%%%%%%%%%%%%

==> pivoter long for arxiv/intro.tex <==
\section{Introduction}\label{sec:intro}
% Pattern counting is an important graph analysis tool in
% many domains: anomaly detection, social network analysis,
% bioinformatics among others [21, 27, 10, 29, 22, 17]. Many
% real world graphs show significantly higher counts of certain
% patterns than one would expect in a random graph [21, 46,
% 27]. This technique has been referred to with a variety of
% names: subgraph analysis, motif counting, graphlet analysis,
% etc. But the fundamental task is to count the occurrence
% of a small pattern graph in a large input graph. In all
% such applications, it is essential to have fast algorithms for
% pattern counting.
% It is well-known that certain patterns capture specific
% semantic relationships, and thus the social dynamics are
% reflected in these graph structures. The most famous such
% pattern is the triangle, which consists of three vertices
% connected to each other. Triangle counting has a rich history
% in the social sciences and network science [21, 46, 10, 47].
% We focus on the more general problem of clique counting.
% A k-clique is a set of k vertices that are all connected to each
% other; thus, a triangle is a 3-clique. Cliques are extremely
% significant in social network analysis (Chap. 11 of [20] and
% Chap. 2 of [23]). They are the archetypal example of a dense
% subgraph, and a number of recent results use cliques to find
% large, dense subregions of a network [32, 41, 28, 43].
Subgraph counting (also known as motif counting, graphlet counting) is a fundamental algorithmic
problem in network analysis, widely applied in domains such as
social network analysis,
bioinformatics, cybersecurity, and physics (refer to tutorial~\cite{SeTi19} and references within).
One of the most important cases is that of \emph{clique counting}. A $k$-clique
is a complete subgraph on $k$ vertices, and has great significance in network analysis
(Chap. 11 of~\cite{HR05} and Chap. 2 of~\cite{J10}).
Indeed, just the special case of $k=3$ (triangle counting) has a rich history in modern
network science. General clique counting has received much attention in recent times
\cite{JhSePi15, MarcusS10,AhNe+15,Escape,JS17,FFF15,DBS18}. There is a line of recent
work on exploiting clique counts for community detection and dense subgraph discovery
\cite{SaSePi14,Ts15,BeGlLe16,TPM17,lu2018community,YiBiKe19}.

% has been of significant interest both to the applied as well as theoretical computer science communities. In the applied world, counts of motifs have been used in social network analysis, in bioinformatics, spam detection, graph modeling~\cite{HoLe70,Milo2002,Burt04,PrzuljCJ04} etc. Clique counting, in particular, has recieved a lot of attention in recent times~\cite{JhSePi15, MarcusS10,AhNe+15,Escape,JS17,FFF15,DBS18}. This is because cliques often have special significance in the context of real-world graphs. For example, a $k-$clique in a social network could point to a group of $k-$friends. The number of $k$-cliques in a graph for different $k$ can be used as a distinguishing feature of a graph which can then be useful in graph generation and modeling. Cliques have also been used in the discovery of dense subgraphs~\cite{SaSePi14,Ts15} , and in community detection ~\cite{lu2018community}. In addition to $k-$clique counts, several applications use per-vertex (and per-edge) $k-$clique counts i.e. the number of $k-$cliques that every vertex ( or edge) is involved in ~\cite{SaSePi14,Ts15}.
%
Despite much effort on this problem, it has been challenging to get scalable algorithms for
clique counting.  
There is a large literature for counting $3$-cliques (triangles) and 
some of these methods have been extended to counting cliques upto size $5$~\cite{JhSePi15, MarcusS10,AhNe+15,Escape}. However, practical algorithms for counting cliques beyond size $5$ have proven to be much harder, and the reason for this is combinatorial explosion. Essentially, as $k$ increases, 
the number of $k$-cliques blows up. 
For large graphs, some recent practical algorithms have succeeded in counting
up to (around) 10-cliques~\cite{FFF15,JS17,DBS18}. They either use randomized approximation
or parallelism to speed up their counting. Besides the obvious problem that they do not scale
for larger $k$, it is difficult to obtain more refined clique counts (such 
as counts for every vertex or every edge).
%     
%     , and these use one of two approaches: either they use parallelization/MapReduce to speed up the counting, or they use randomised approaches to obtain approximate answers. Both these approaches are not suitable for large $k$ and end up requiring huge amounts of space and/or time. Obtaining $k-$clique counts is difficult, obtaining per-vertex and per-edge $k-$clique counts is even more so. Thus, there is a need for practical algorithms that can count larger cliques.
% 
\begin{figure*}[t!]
    % \begin{subfigure}[b]{0.5\textwidth}
    % \centering
    % \includegraphics[width=\textwidth]{Figures/percent_relative_error_k=7.pdf}
    %     \caption{\footnotesize{Timings}}
    %     \label{fig:timings}
    % \end{subfigure}
% ~

\begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/timings-big4-maxk.pdf}{}
    \caption{\footnotesize{Timings}}
    \label{fig:timings}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/as-skitter-occurrences.pdf}{}
    \caption{\footnotesize{Frequency distribution}}
    \label{fig:soc-pokec-occurrences}
    \end{subfigure}
~
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/web-Stanford-occurrences-5.pdf}{}
    \caption{\footnotesize{Frequency distribution}}
    \label{fig:web-Stanford-occurrences}
    \end{subfigure}

    % \hfill
    


            \caption{\Fig{timings} shows the comparison of time taken (in seconds) by \mainalg{} for 4 of our largest graphs to count \textit{all} $k-$cliques with the time taken by kClist40 (the parallel version of the state of the art algorithm kClist that uses 40 threads) to count the number of $k-$cliques, where $k$ is the maximum clique size in each graph. For Stanford, BerkStan, as-skitter, orkut, the maximum clique sizes were 61, 201, 67 and 51 resp. \mainalg{} terminated for most graphs in minutes, (except for orkut, for which it took about 2 hours) whereas kClist40 had not terminated even after 3 days, giving a speedup of 100x to 10000x. \Fig{timings} also shows the time taken by \mainalg{} to obtain the per-vertex and per-edge $k-$clique counts. They were within a factor of the time taken to obtain global $k-$clique counts. \Fig{soc-pokec-occurrences} and  \Fig{web-Stanford-occurrences} shows the frequency distribution of $k$-cliques i.e. for every number $r$ on the x-axis, the y-axis shows the number of vertices that participate in $r$ $k$-cliques, for $k \in [5, 10, 15, 20, 25]$ for as-skitter and web-Stanford graphs. } 
        % \label{fig:comparison}
% ~
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     % \includegraphics[width=\textwidth]{Figures/speedup_k=7.pdf}
%         \caption{\footnotesize{Number of recursive calls}}
%         \label{fig:num-calls}
%     \end{subfigure}
    % \caption{ Summary of behavior of \mainalg{} over several datasets. \Fig{acc} shows the percent relative error in the estimates for k=7 given by \mainalg{}. We only show results for graphs for which we were able to obtain exact counts using either brute force enumeration, or from the results of~\cite{FFF15}. The errors are always $<2\%$ and mostly $<1\%$. \Fig{timings} shows the time taken by \mainalg{} for k=7 and k=10. \Fig{7-speedup} shows the speedup (time of algorithm/time of \mainalg) over other state of the art algorithms for k=7. The red line indicates a speedup of 1. We could not give a figure for speedup for k=10 because for most instances no competing algorithm terminated in min(7 hours, 100 times \mainalg{} time).}
\end{figure*}


% From a theoretical standpoint, the best known algorithm for counting $k-$cliques runs in time $n^{\theta(k)}$ whereas the best known algorithm for counting all cliques is the trivial algorithm that runs in time $O(2^n)$ for an $n-$vertex graph. 
% \Shweta{Consider whether to talk about the approximation algorithms like Talya's recent paper here.}

% \begin{enumerate}
%     \item Clique counting very important
%     \item problem very hard
% \end{enumerate}

\subsection{Problem Statement} \label{sec:problem}

We are given an undirected, simple graph $G(V,E)$. For $k \geq 3$, a $k$-clique 
is a set of $k$ vertices that induce a complete subgraph (it contains all edges
among the $k$ vertices). We will denote the number of $k$-cliques as $C_k$.
For a vertex $v \in V$, we use $c_k(v)$ to denote the number of $k$-cliques
that $v$ participates in. Analogously, we define $c_k(e)$ for edge $e \in E$.

We focus on the following problems, in increasing order of difficulty. 
We stress that $k$ is \emph{not} part
of the input, and we want results for all values of $k$.

\begin{asparaitem}
    \item Global clique counts: Output, $\forall k \geq 3$, $C_k$.
    \item Per-vertex clique counts: Output, $\forall k$, $\forall v \in V$, the value $c_k(v)$.
    \item Per-edge clique counts: Output, $\forall k$, $\forall e \in E$, the value $c_k(e)$.
\end{asparaitem}

The per-vertex and per-edge counts are sometimes called \emph{local counts}.
In clustering applications, the local counts
are used as vertex or edge weights, and are therefore even more
useful than global counts~\cite{SaSePi14,Ts15,BeGlLe16,TPM17,lu2018community,YiBiKe19}.

\medskip


\textbf{Challenges:} Even the simplest problem of getting global 
clique counts subsumes a number of recent results on clique counting
\cite{FFF15,JS17,DBS18}. The main challenge
is combinatorial explosion: for example, the {{\tt web-Stanford}} web graph
with 2M edges has \emph{3000 trillion} $15$-cliques. These numbers are even
more astronomical for larger graphs. Any method that tries to enumerate
is doomed to failure. 

Amazingly, recent work by Danisch-Balalau-Sozio
uses parallel algorithms to count beyond trillions of cliques.
But even their algorithm fails to get all global clique counts for a number
of datasets. Randomized methods
have been used with some success, but even they cannot estimate
all clique counts~\cite{FFF15,JS17}.

Local counting, for all $k$, is even harder, especially given the sheer
size of the output. Parallel methods would eventually need to store
local counts for every subproblem, which would increase the overall memory footprint.
% the final local counts, which could create bottlenecks.
For local counts, sampling would require far too many random variables, each of which
need to be sampled many times for convergence.
(We give more explanation in \Sec{related}.)

This raises the main question:

{\em Is there a scalable, exact algorithm for getting all global and local cliques counts,
on real-world graphs with millions of edges?} 

To the best of our knowedge, there is no previous algorithm that can solve these problems
on even moderate-sized graphs with a few million edges. 

% In addition to the number of $k-$cliques, we also want to provide the per vertex $k-$clique counts (i.e. for every vertex in the graph and every possible $k$, what is the number of $k-$cliques that the vertex is a part of) and the per-edge $k-$clique counts (i.e. for every edge in the graph and every possible $k$, what is the number of $k-$cliques that the edge is a part of).
% 
% It is important to distinguish $k-$cliques from maximal $k-$cliques. A maximal $k-$clique is a $k-$clique that cannot be extended further. 

% \subsection{Challenges} \label{sec:challenges}
% Exact counting algorithms focus on 



\subsection{Main contributions} \label{sec:contri}
Our main contribution is a new practical algorithm \mainalg{} for the global and local clique counting
problems. 

\textbf{Exact counting without enumeration:} Current methods for exact clique counting
perform an \emph{enumeration}, in that the algorithm explicitly ``visits" every clique. Thus,
this method cannot scale to counting larger cliques, since the number of cliques is simply too large.
Our main insight is that the method of \emph{pivoting}, used  
to reduce recursion trees for maximal clique 
enumeration~\cite{BK73,ELS13}, can be applied to counting cliques of all sizes. 

\textbf{Succinct Clique Trees through Pivoting:} We prove that pivoting can be used
to construct a special data structure called the \emph{Succinct Clique Tree} (SCT).
The SCT stores a unique representation of all cliques, but is much smaller than
the total number of cliques. It can also be built quite efficiently.
Additionally, given the tree, one can easily ``read off" the number of $k$-cliques 
and various local counts in the graph. Remarkably, we can get all counts without storing the entire tree and the storage required at any point is linear in the number of edges. 

%  This is a non-trivial
% result, since maximal cliques can overlap arbitrarily and it is not clear how to extract
% all $c_k$s from only maximal cliques. \Shweta{We apply pivoting to the enumeration tree and notice that we not only reduce the tree drastically, but can efficiently count without explicitly producing all cliques.}
% 
% Formally, we build off the implementation
% of the classic Bron-Kerbosch maximal clique algorithm~\cite{BK73}, by Eppstein-L\"{o}effler-Strash
% \cite{ELS13}. We prove that by carefully looking at the recursion tree of that algorithm,
% one can compute all global and local $k$-clique counts. \Shweta{this isn't quite true. Needs change.}
% Remarkably, this can be done efficiently without explicitly producing all cliques. 
% For global clique counts, the extra overhead is negligible.

% We prove that a carefully 
% overlaid scheme for differentiating vertices in the recursion tree, and counting cliques based on this scheme can yield the counts of all $k$-cliques. 
%
\textbf{Excellent practical performance:} We implement \mainalg{} on a commodity machine.
For global clique counting, \mainalg{} is able to process graphs of up to tens of millions
of edges in \emph{minutes}. Previous results either work only for small values of $k$ (typically up to $10$) or take much longer.
Consider \Fig{timings}, where the time of \mainalg{} is compared
with that of kClist (the state of the art parallel algorithm for clique counting)~\cite{DBS18}. 
In the instances shown kClist did not terminate even after running for 3 days. By
contrast, for the largest {\tt com-orkut} social network with
more than 100M edges, \mainalg{} gets all values of $C_k$ within two hours.
(Typically, in this time, kClist gets $k-$clique counts only up to $k \leq 13$.)
% We stress
% that kClist only computes $c_k$ for some chosen value of $k$ (we set $k = 13$, the largest
% our machine could handle \Shweta{for the large graphs}). \mainalg{} is computing all values of $c_k$. Nonetheless, \mainalg{}
% is actually faster for larger graphs. For the largest {\tt com-orkut} social network with
% more than 100M edges, \mainalg{} \Shweta{counts k-cliques for all k} within two hours.

\textbf{Feasible computation of local counts:} \mainalg{} is quite efficient for per-vertex counts, and runs
in at most twice the time for global counts. The times for local clique counting
are given in \Fig{timings}. Even for the extremely challenging problem
of per-edge counts, in most instances \mainalg{} gets these numbers in a few hours.
(For the {\tt com-orkut} social network though, it takes a few days.) 

This allows us to get data shown in \Fig{soc-pokec-occurrences} and \Fig{web-Stanford-occurrences}, 
that plots the frequency distribution
of $k$-cliques. (In other words, for every number $r$, we plot the number of vertices
that participate in $r$ $k$-cliques.) As mentioned earlier, this information is
used for dense subgraph discovery~\cite{SaSePi14,Ts15}. 
To the best of our knowledge, this is the first algorithm that is able to get
such information for real-world graphs. 
% \mainalg{} makes local clique counting feasible. 

% \textbf{Theoretical running time analysis of \mainalg:} We do not consider this our primary
% contribution, but we can formally prove that \mainalg{} gets all global counts
% in time $O(n3^{\alpha/3})$.
% Here, $\alpha$ is the graph degeneracy, alternately called the maximum core number. This
% follows from standard techniques in the analysis of pivoting for maximal clique enumeration
% by Tomita et al and Eppstein-Strash~\cite{Tomita04,ES11}.
% 
% Until now, algorithms for counting all cliques have essentially enumerated all cliques ~\cite{FFF15, DBS18}. In a graph titled web-BerkStan (a graph with 0.6M nodes and 6.6M edges obtained from SNAP~\cite{Snap}  representing the pages from the stanford.edu and berkeley.edu domains), there are $1.1*10^{59}$ 105-cliques. Enumerating these cliques is not a practical option, if not impossible. \mainalg{} uses the reduced recursion tree of \BK{} to count all cliques without enumerating them. \Fig{comparison} shows a comparison of the time taken by the state-of-the-art \textbf{parallel} algorithm called kClist with \mainalg{}. kClist40 takes as input a $k$ and using 40 threads enumerates (and thus outputs the number of) $k-$cliques. \mainalg{} does not take $k$ as input but rather outputs for all $k$ in a single run. As shown in \Fig{comparison}, \mainalg{} obtains counts of \textbf{all} $k-$cliques in a fraction of the time taken by kClist to obtain counts of $13-$cliques. For the web-BerkStan graph, \mainalg{} counted all cliques in 25 seconds whereas kClist did not terminate even after 3 days. The largest clique in the graph is of size 201. The largest clique size that state of the art methods have been able to count in these graphs is 29 ~\cite{DBS18}. Thus, \mainalg{} for the first time is able to give counts of cliques which no other algorithm was able to before, despite using parallelization. Indeed, the plot in \Fig{trends} has been achieved for the first time.


 
% \textbf{Enhances a classic algorithm:} \mainalg{} is based on the pivoted version of the classic Bron-Kerbosch~\cite{BK73} algorithm which is a recursive algorithm for maximal clique counting proposed in 1973 (henceforth known as \BK{}). Other maximal clique counting algorithms essentially enumerate all cliques and check if they are maximal, while \BK{} uses a heuristic to massively cut down the search space, and is known to work very well in practice. However, since maximal cliques can overlap in arbitrary ways, it is not obvious how one can efficiently extract the counts of all $k-$cliques from the set of maximal cliques. % \mainalg{} also 
 % In other words, it has a much smaller recursion tree (building which takes the bulk of the time) and \mainalg{} benefits from this reduced recursion tree. \mainalg{} has important implications both from the practical as well as theoretical standpoints. 

% \Shweta{Should we have a plot here about the size of recursion tree in our case vs in Max's case?}



% Based on these trend there was no hope for being able to count larger cliques before \mainalg{} despite using parallelization and MapReduce. 

% \Fig{timings} shows the time taken by \mainalg{} to count all cliques in some real-world graphs.

% \Fig{num-calls} shows the number of calls made by enumeration algorithms and the number of calls made by \mainalg{}. \mainalg{} results in a much smaller tree and as a result, \mainalg{} is able to count all cliques in a fraction of the time taken by other state of the art algorithms. 

% \textbf{Obtains all per vertex and per edge $k-$clique counts:} In addition to obtaining $k$-clique counts, \mainalg{} also provides per vertex and per edge $k-$clique counts, using only slightly more time. Because our algorithm is sequential, we only need to maintain one copy of the data structure that collects the counts. On the other hand, parallel algorithms would either need to update the data structure sequentially (which would slow it down considerably) or need to maintain multiple copies of the data structure (one per thread). Since the data structure for storing per vertex and per edge $k-$clique counts can become very large, maintaining multiple copies of it could potentially take a prohibitively large amount of memory.  \mainalg{} is extremely fast while still being sequential, thus bypassing this problem.

% \textbf{$O(3^{\frac{n}{3}})$ algorithm:} Incidentally, \mainalg{} also improves the theoretical bound for the time complexity of clique counting. The worst case time complexity of clique enumeration is $O(2^n)$. As Eppstein et. al showed, the worst case running time of \BK{} is $O(3^{n/3})$ and this carries over to \mainalg{}, thus giving a theoretically as well as practically much faster algorithm for clique counting.

% \textbf{Obtains all per edge clique counts:}

% \textbf{Obtains trends in clique counts:} For many of the real world graphs, for the first time we are able to look at trends in clique counts and the entire clique distribution. This opens the door for newer insights and analysis tools using clique counts. 

\subsection{Related Work} \label{sec:related}

Subgraph counting has an immensely rich history in network science, ranging from applications
across social network analysis, bioinformatics, recommendation systems, graph clustering
(we refer the reader to the tutorial~\cite{SeTi19} and references within). We only
describe work directly relevant to clique counting.

The simplest case of clique counting is \emph{triangle counting}, which has 
received much attention from the data mining and algorithms communities. Recent work
has shown the relevance of counts of large subgraphs (4, 5 vertex patterns)
~\cite{BeHe+11,UganderBK13,SGB16,RKKS17,YiBiKe18}. Local clique counts
have played a significant role in a flurry of work on faster and better algorithms
for dense subgraph discovery and community detection~\cite{SaSePi14,Ts15,BeGlLe16,TPM17}.
The latter results define the ``motif conductance", where cuts are measured by the
number of subgraphs (not just edges) cut. This has been related to higher order
clustering coefficients~\cite{YiBiKe18,YiBiKe19}. These quantities
are computed using local clique counts, underscoring the importance of these numbers.

The problem of counting cliques (and variants such as counting maximal cliques) has received much attention 
both from the applied and theoretical computer science communities~\cite{ChNi85,AlYuZw94,CHKX04,V09}.
Classic techniques like color-coding~\cite{BetzlerBFKN11,ZhWaBu+12} and
path sampling~\cite{SePiKo14,JhSePi15,WaZh+18} have been employed for counting cliques up to size $5$.

For larger cliques, Finocchi-Finocchi-Fusco gave a MapReduce algorithm that uses
orientation and sampling techniques~\cite{FFF15}. Jain and Seshadhri
use methods from extremal combinatorics to give a fast sampling algorithm~\cite{JS17},
that is arguably the fastest approximate clique counter to date. In a remarkable
result, Danisch-Balalau-Sozio gave a parallel implementation (kClist) of a classic algorithm
of Chiba-Nishizeki, which is able to enumerate upto trillions of cliques~\cite{DBS18}.
For exact counting, we consider kClist as the state of the art.
Despite the collection of clever techniques, none of these methods really scale beyond
counting (say) 10-cliques for large graphs.

\textbf{Why local counting is hard:} Note that either parallelism or sampling is used to tame the combinatorial explosion.
Even though (at least for small $k$), one can enumerate all cliques in parallel, local
counting requires updating a potentially global data structure, the list
of all $c_k(v)$ or $c_k(e)$ values. To get the benefits of parallelism, one would 
either have to duplicate a large data structure or combine results
for various threads to get all local counts. While this may be feasible, it
adds an extra memory overhead. 

Sampling methods typically require some overhead for convergence. For local counts,
there are simply too many samples required to get accurate values for (say) all $c_k(v)$ values.
For these reasons, we strongly believe that new ideas were required to get efficient
local counting.

\textbf{Maximal clique enumeration:} Extremely relevant to our approach is a line
of work of maximal clique enumeration. A \emph{maximal clique}
is one that is not contained in a larger clique. Unlike the combinatorial explosion
of $k$-cliques, maximal cliques tend to be much fewer. The first algorithm for this problem
is the classic Bron-Kerbosch backtracking procedure from the 70s~\cite{BK73,A73}.
They also introduced an idea called \emph{pivoting}, that prunes the recursion tree for
efficiency.
Tomita-Tanaka-Takahashi gave the first theoretical analysis of pivoting rules,
and showed asymptotic improvements~\cite{Tomita04}. Eppstein-L\"{o}effler-
Strash
combined these ideas with orientation methods to give a practical and provably fast
algorithm for maximal clique enumeration~\cite{ES11,ELS13}. An important empirical
observation of this line of work is that the underlying recursion tree created with pivoting
is typically small for real-world graphs. This is the starting point 
for our work.

% To make clique counting feasible for very large grapsh, randomized approaches like color-coding~\cite{AlYuZw94,BetzlerBFKN11,ZhWaBu+12}, edge sampling ~\cite{TsKaMiFa09,TsKoMi11,RaBhHa14}, MCMC ~\cite{BhRaRa+12} based methods have been proposed but they don't scale well~\cite{JhSePi15}. Starting with the seminal work of Bron-Kerbosch~\cite{BK73}, the problem of counting maximal cliques has been studied also from a practical standpoint ~\cite{A73,Tomita04,ES11}. Methods for finding the maximum clique using branch and bound methods have also been proposed~\cite{RossiG15}.
% 
% 
% 
% Even though pattern counting as a tool for graph analysis has been mentioned in literature as early as the 70's ~\cite{HoLe70, Sh71}, it was the seminal work of Milo {\em et al.}~\cite{Milo2002}  that brought attention to it. They used network motifs (also known as patterns, graphlets) to distinguish real-world graphs from random graphs. Subsequently, similar to the vertex degree distribution, ~\cite{MilenkovicP08} and ~\cite{ShVi+09} defined a graphlet degree distribution and graphlet kernel, respectively as tools to compare graphs. 
% 
% The use of triangles, and clustering coefficients in particular, has a rich history. Triangle counts have been used in spam detection~\cite{BeBoCaGi08} and role detection~\cite{Burt04}. ~\cite{SaCa+10} uses clustering coefficients (among other properties) to show that Preferential Attachment has poor clustering. ~\cite{SeKoPi11,SonKanKim12,PfFo+12} use triadic closure properties to model graphs. Several algorithms for counting triangles in different setups (streaming, temporal, distributed) have been proposed ~\cite{ArKhMa12,BeBoCaGi08,BuFrLeMaSo06,JhSePi13}. The past decade saw use of 4 and 5 vertex patterns ~\cite{UganderBK13,BeHe+11} in graph analysis. ~\cite{YiBiKe18} define higher order clustering coefficients for cliques beyond size 3. Cliques being dense substructures, have found applications in dense subgraph discovery 
% algorithms~\cite{SaSePi14,Ts15} and in topological approaches to network analysis~\cite{SGB16}. 
% 
% ~\cite{JhSePi15, MarcusS10,AhNe+15,Escape} give efficient ways to count patterns upto size 5. The first work to give a practical algorithm for counting cliques beyond size 5 is a MapReduce algorithm of Finocchi {\em et al.} ~\cite{FFF15}. ~\cite{JS17} provide a randomized algorithm to count cliques upto size 10. The closest to our work is that of ~\cite{DBS18} which is the state-of-the-art parallel algorithm that enumerates (and hence counts) all cliques. We will do a detailed comparison with these methods in the evaluation section.
% 
% From an algorithmic perspective, clique counting has received
% much attention from the theoretical computer science community~\cite{ChNi85,AlYuZw94,CHKX04,V09}.
% Maximal clique enumeration has been an important topic~\cite{A73,Tomita04,ES11} since
% the seminal algorithm of Bron-Kerbosch~\cite{BronKerb73}. Practical
% algorithms for finding the maximum clique were given by Rossi {\em et al.} using
% branch and bound methods~\cite{RossiG15}.

% Most relevant to our work is a classic algorithm of Chiba and Nishizeki~\cite{ChNi85}.
% This work introduces graph orientations to reduce the search time and provides
% a theoretical connection to graph arboricity. We also apply this technique in \mainalg.

% The closest result to our work is a recent MapReduce algorithm of Finocchi {\em et al.} 
% for clique counting~\cite{FFF15}. This result applied the orientation technique of~\cite{ChNi85},
% and creates a large set of small (directed) egonets. Clique counting overall 
% reduces to clique counting in each of these egonets, and this can be parallelized using MapReduce.
% We experiment on the same graphs used in~\cite{FFF15} (particularly, the largest ones)
% and get accurate results on a single, commodity machine (as opposed to using a cluster).
% Alternate MapReduce methods using multi-way joins have been proposed,
% though this is theoretical and not tested on real data~\cite{AFRATI13}.

% A number of randomized techniques have been proposed for pattern counting,
% and can be used to design algorithms for clique counting. Most prominent
% are color coding~\cite{AlYuZw94,HoBe+07,BetzlerBFKN11,ZhWaBu+12}
% and edge sampling methods~\cite{TsKaMiFa09,TsKoMi11,RaBhHa14}. (MCMC methods~\cite{BhRaRa+12}
% typically do not scale for graphs with millions of vertices~\cite{JhSePi15}.)
% We perform detailed comparisons with these methods, and conclude that they
% do not scale for larger clique counting.

% we merely point
% to the related work of~\cite{TsKoMi11,SePiKo13} for more details.
% 
% . It has since found many applications including in graph modeling ~\cite{PrzuljCJ04,HormozdiariBPS07}, graph comparisons ~\cite{PrzuljCJ04,HalesA08}  among others. Triangle counting, especially, have been extensively studied under different scenarios. (see related work sections of ~\cite{TsKoMi11,SePiKo13}.)
% 
% Other variants of clique-counting, including maximum clique enumeration and maximal clique counting have also received considerable attention. Most of the techniques used for finding the maximum cllique, including in the recent work of ~\cite{RossiG15} involve using a branch and bound approach to prune the search space for the maximum clique. For finding maximal cliques, ~\cite{BronKerb73} gave the first exact algorithm, which was subsequently optimized and analyzed by ~\cite{Tomita04}.
% 
% The problem of finding all cliques differs fundamentally from the above two because the number of k-cliques goes up exponentially with k. ~\cite{CHIBAN85} gave one of the first exact algorithms for counting cliques. It works by  ordering the vertices and doing an edge search to check if the new vertex obtained by adding an adge to an already found clique, results in a bigger clique. Ordering avoids finding each clique multiple times and ensures that each clique is found exactly once. In this way, it finds all cliques. However, it does not exploit the community-structure of real-world graphs. 
% % \Shweta{Actually, isn't this the algorithm that we are calling "naive enumeration" or "brute force enumeration"?}
% 
% Another approach to address the problem is through the use of parallel algorithms. \cite{AFRATI13} and more recently, \cite{FiFiFu14} gave parallel algorithms for counting cliques using MapReduce. While the former uses multi-way joins as its basic building block to give a one-round algorithm to count cliques, the latter gives a 3-round algorithm that computes the out-neighborhood of each node and counts k-1-cliques within each neighborhood. It should be noted that the time required to find the exact count using this algorithm and specialized MapReduce hardware is comparable to our algorithm which gives approximate counts within $1\%$ using only commodity hardware.
% 
% Getting the exact count of cliques is often an overkill as approximate counts suffice, as in the case of ~\cite{UganderBK13}. Several algorithms have been proposed which use sampling for getting approximate counts: Edge Sampling, GRAFT, ColorCoding. Indeed, ~\cite{FiFiFu14} also propose a sampling scheme given for estimating the counts using MapReduce - using one of the color-coding or edge sampling based methods to estimate the number of cliques in each out-neighborhood. Both these sampling methods do not scale well with clique size, as we shall see in \Sec{results}.  This is because the expected number of cliques of these methods goes down with k, thus increasing the variance of the estimates. 
% % \Shweta{Should have a plot for this, showing how other methods perform in terms of accuracy for 2 different clique sizes}
% 
% If we repeat the 3 rounds of the parallel algorithm until each out-neighborhood becomes dense, and sample within each such dense neighborhood, then that would be the parallel version of our algorithm. Importantly, they note that counting the $k-1$-cliques takes much more time than the 3 rounds to compute the out-neighborhoods. This is where we believe our algorithm can help. By doing multiple rounds of the inexpensive steps to boost the density of cliques in the resulting out-neighborhoods, we reduce the variance at a small price. 
% 
% We will use Edge Sampling, GRAFT, ColorCoding and naive enumeration algorithm to compare our algorithm with.
% 
% {\it Brute force enumeration}: Brute force enumeration works by converting the graph into a DAG by ordering the vertices and then counting the number of k-cliques with each node as the smallest rank node. This makes sure that every clique is reported exactly once.
% 
% {\it Edge Sampling \Shweta{Sesh, please cite}:} This method uses a Markov Chain Monte Carlo (MCMC) based method to uniformly sample a clique of a paticular size from the space of all cliques of that size. We can think of this as down-smapling the edges of the graph, keeping an edge with a constant probability, and appropriately scaling the number of cliques in the resultant graph.
% 
% {\it  GRAFT~\cite{RaBhHa14}:} This algorithm samples a set of edges uniformly at random and then counts the number of cliques incident on each edge. The average number of cliques so obtained is scaled by the number of edges to get an unbiased estimate for the total number of cliques of a given size in the input graph. 
% %(A motif with $i$ edges may be counted $i$ times but the final count can be adjusted by accounting for this over counting.) 
% % Observe that if edges are sampled with probability 1, this gives an algorithm for exact counting using an edge iteration.  
% 
% {\it Color Coding~\cite{AlYuZw94,HoBe+07,BetzlerBFKN11,ZhWaBu+12}:} This is a commonly used technique for pattern counting. It works by asigning a color out of k colors to every vertex, uniformly at random. We then enumerate all k-cliques that have distinct colors and scale them appropriately to get unbiased estimates of total k-cliques in the input graph.
% For our experiments, for estimating k-cliques we used k colors and used the same enumeration algorithm described above. 
% 
% We have used our own implementations for all 4 methods. As the results of our detailed study shows, these algorithms do not scale well. For a web-network between Berkeley and Stanford (web-BerkStan), \mainalg took less than 4 minutes to find all cliques of size 10, where all the other algorithms took more than 3 hours to achieve similar or worse accuracy as \mainalg. 
% 
% Triangle counting has been extensively explored in various setups (see related work sections of ~\cite{TsKoMi11,SePiKo13}.)
% check in parallel algo paper for references

% Motif counting for bioinformatics was arguably initiated by a 
% seminal paper of Milo {\em et al.}~\cite{Milo2002}. This technique has been
% used for graph modeling~\cite{PrzuljCJ04,HormozdiariBPS07}, graph comparisons~\cite{PrzuljCJ04,HalesA08}, and even decomposing a network~\cite{Itzkovitz_2005}.
% %
%One of the first works to emphasize significance of motif counting in bioinformatics is the seminal work of Milo {\em et al.}~\cite{Milo2002}. Since then there have been many further works. For example, Przulj {\em et al}~\cite{PrzuljCJ04} use motifs distribution to argue that protein-protein interaction networks resemble a particular network model than previously thought. Similarly, in \cite{HormozdiariBPS07}, motifs distribution is described as an important characteristic for evaluating network models. Hales and Arteconi~\cite{HalesA08} found that motifs profile of peer-to-peer networks resemble protein networks. Similarly, motif counts has been used for hierarchal network decomposition~\cite{Itzkovitz_2005}. 
% Refer to \cite{BetzlerBFKN11,WongBQH12} for more details. 

% Triangle counting has a rich history in social sciences and related analyses, that
% we simply refer the reader to the related work sections of~\cite{TsKoMi11,SePiKo13}.
% The significance of 4-vertex patterns was studied in recent work of Ugander et al.~\cite{UganderBK13},
% who propose a ``coordinate system'' for graphs based on the motifs distribution. This is used
% for improved network classification, and the input graphs were comparatively small (thousands of vertices).

% Previous studies tailored to 4-vertex patterns~\cite{GonenS09,MarcusS10} provide both exact and approximation algorithms. These are limited to small graphs. For example, a graph with 90K edges
% requires 40 minutes of processing~\cite{MarcusS10} (on a single machine).

% Most relevant to this work are previous studies on \emph{wedge sampling}~\cite{ScWa05-2,SePiKo13,KoPiPlSe13}. This method samples paths of length 2 to estimate
% various triangle statistics. Our method of 3-path sampling can be seen as building
% on wedge sampling. But we require new techniques of path pruning to get the algorithm
% to work accurately. These pruning techniques are inspired by degeneracy ordering algorithms
% for triangle counting~\cite{ChNi85,ScWa05}.
% We can actually provide mathematical error bars for real
% runs and instances (as opposed to just a theoretical proof of convergence of estimate).


% \subsection{Community structure and intuition behind the algorithm}
% It has been well documented that most real-world graphs exhibit community-structure. \cite{GiMiNe02} What this means is that the edges of the graph, instead of being strewn randomly all over the graph (as one would expect in a random graph), tend to be concentrated in possibly overlapping, dense pockets. Consider for example, the Facebook graph. One would typically expect to see dense communities corresponding to different organizations and groups but relatively fewer connections across the groups. This is the structure that our algorithm exploits.
% In a graph with n vertices, there could potentially be ${n \choose k}$ k-cliques. Essentially what a sampling algorithm for cliques intends to find is: what is the probability that a randomly picked set of k-vertices forms a clique? Since most real-world graphs are sparse, answering this question by sampling on the large sparse graph would require a very large number of samples. Instead, if we drill down on the dense regions and look for cliques within these dense regions, then a much smaller number of samples suffices, and this is where the community structure of graphs helps. 
% 
% We can think of our experiment being analogous to an experiment to estimate the probability of a biased coin coming up heads. The number of samples (coin flips) required to accurately estimate the probability decreases as this probability increases. Thus, by drilling down on the dense regions in the graph quickly, we are reducing the search space dramatically and boosting the success probability of our experiment, resulting in the algorithm requiring far fewer samples.
% 
% The Tur\'{a}n density of a graph gives us the maximum density a graph can have without having a k-clique~\cite{TURAN41}. Erd\H{o}s ~\cite{ErdSimo83} proved that if a graph has even 1 more edge that given by the above density, then it must contain many k-cliques. The Lovasz-Simonovitz bound tells us that if the density of a graph is sufficiently larger than the density, then a constant fraction of k-node sets form k-cliques. In other words, a constant number of samples suffice to estimate the proportion of k-cliques in the graph. By ensuring that we drill down until every sub-graph has density greater than the Tur\'{a}n  density, we put a bound on the number of samples needed to accurately estimate the number of k-cliques. 
% 
% \subsection{Comparison with previous work}

% We give a more detailed history of previous work in \Sec{related}. Here, we highlight the difference
% from previous results on subgraph counting. The work (beyond triangle counting)
% involves color coding methods~\cite{HormozdiariBPS07,BetzlerBFKN11,ZhWaBu+12}, MCMC based sampling
% algorithms~\cite{BhRaRa+12}, incremental pattern building algorithms
% for Map-Reduce~\cite{Pl12,BhHa13} edge sampling algorithms~\cite{RaBhHa14}.

% Our main contribution is the fact that we provide a generic framework that can be used to calculate the clique counts for a range of clique sizes. 
% The differences between the above methods and the new algorithm are highlighted below.

% \begin{asparaitem}%[\IEEEsetlabelwidth{This must be good}]
% \item[\textbf{Scalability and speed.}] Previous work either employ Map-Reduce clusters
% or max out at a million (or so) edges. Our algorithm runs on a single commodity machine
% with 64GB memory, and easily handles graphs with more than a hundred million edges.
% No previous result can get such scalability for clique counting (Note: Check this statement).
% \item[\textbf{Accuracy.}] Our algorithm's accuracy is both empirical and provable. 
% Previous methods~\cite{BhRaRa+12} for motif analyses get the frequencies correct up to an order of magnitude. Our relative errors 
% of $1\%$ are much smaller than any of the previous results we are aware of. Furthermore, we can explicitly
% put realistic error bars on all our estimates. Again, this distinguishes our algorithm
% from the state of the art.
% \item[\textbf{Comprehensive results for small clique counts.}] We get detailed results
% for all small cliques on a large number of graphs, and believe this is useful for further data analysis
% (as done in~\cite{UganderBK13}). Previous work usually focuses on a small, specific 
% set of larger motifs~\cite{HormozdiariBPS07,BetzlerBFKN11,ZhWaBu+12}, or gives coarser approximations
% for more motifs~\cite{BhFRaRa+12}.
% \end{asparaitem}




==> pivoter long for arxiv/results.tex <==
{\bf Preliminaries:} All code for \mainalg{} is available here: \href{https://bitbucket.org/sjain12/pivoter/}{https://bitbucket.org/sjain12/pivoter/}. We implemented our algorithms in C
and ran our experiments on a commodity machine equipped
with a 1.4GHz AMD Opteron(TM) processor 6272 with 8 cores and
2048KB L2 cache (per core), 6144KB L3 cache, and 128GB
memory.
We performed our experiments on a collection of social networks, web networks, and
infrastructure networks 
from SNAP [49]. 
The graphs are simple and undirected (for graphs that are directed, we ignore the direction).
A number of these graphs have more than 10 million edges, and the largest has more than
100 million edges.  Basic properties of these graphs are presented in \Tab{main}. 

The data sets are split into two parts, in \Tab{main}. The upper part are
instances feasibly solved with past work (notably kClist40~\cite{DBS18}), while
the lower part has instances that cannot be solved with previous algorithm (even
after days). We give more details in \Sec{time}.

{\bf Competing algorithms:} We compare with (what we consider) are the state
of the art clique counting algorithms: Tur\'{a}n-Shadow (TS)~\cite{JS17} and kClist40~\cite{DBS18}.

\textbf{kClist40:} This algorithm by Danisch-Balalau-Sozio~\cite{DBS18} uses 
degeneracy orientations and parallelization to enumerate all cliques. 
The kClist40 algorithm, to the best of our knowledge, is the only existing algorithm
that can feasibly compute all global counts for some graphs. Hence, our main focus
is runtime comparisons with kClist40.

We note that the implementation of kClist40 visits every clique, but only
updates the (appropriate) $C_k$. While it could technically compute local counts,
that would require more expensive data structure updates. Furthermore, there would
be overhead in combining the counts for independent threads, and it is not
immediately obvious how to distribute the underlying data structure storing
local counts. As a result, we are
unaware of any algorithm that computes local counts (at the scale of dataset in \Tab{main}).

We perform a simple optimization of kClist40, to make counting faster.
Currently, when kClist40 encounters a clique, it enumerates every smaller clique contained inside it. 
For the purpose of counting though, one can trivially count all subcliques
of a clique using formulas. We perform this optimization (to have a fair comparison with kClist40),
and note significant improvements in running time.

In all our runs, for consistency, we run kClist with 40 threads. 
Note that we compare the \emph{sequential} \mainalg{} with the \emph{parallel} kClist40.

\textbf{TS:} This is an approximate clique counting algorithm for $k$ upto $10$ ~\cite{JS17}. 
It mines dense subgraphs (shadows) and samples cliques within the dense subgraphs
to give an estimate. For fast randomized estimates, it is arguably the fastest algorithm.
It runs significantly faster than a sequential implementation of kClist, but is typically comparable
with a parallel implementation of kClist.
It requires the entire shadow to be available for sampling which can require considerable space. 
% 
%  as one could simply get the number of smaller cliques contained inside a clique by calculating ${n \choose k}$ where $n$ is the size of the clique and $k<n$ is the size of smaller clique. So we optimize their algorithm and indeed, in some cases we see significant improvement in the running time. 
% 
% 
% 
% Note however that in the implementation provided by the authors, they do not list every clique but simply update the count of $k-$cliques. Although the algorithm in principle can provide per-vertex and per-edge $k-$clique counts, the algorithm would run into the same problem as we did in the parallelization of \mainalg{}, namely that the replication of result data structures can take up a lot of memory. Hence, we feel the right comparison of kClist with \mainalg{} should be with the parallel version of \mainalg{} that simply counts all $k-$cliques. 
% 
% 
% The authors also do a detailed study of the runtimes of the Chiba-Nishizeki algorithm ~\cite{ChNi85} (on which their clique enumeration algorithm is based), the sequential version of their algorithm (kClist) and 2 parallel versions kClistNodeParallel and kClistEdgeParallel. The authors show that out of all the different variants they experimented with, kClistEdgeParallel with 40 threads (abbreviated to kClist40) gives the best performance and we will use this for comparison. Note that  kClist40 is the only algorithm that attempts to count cliques beyond size 10 that does not require Map-Reduce or any specialized hardware. The algorithm lists every clique. For any results listed for kClist40 in this paper we use this optimization. Note that \mainalg{} algorithm can easily be used for listing all cliques, however we consider that out of the scope of this paper and focus on counting. 
% 



\subsection{Running time and comparison with other algorithms} \label{sec:time}

\textbf{Running time for global counting:} We show the running time results in \Tab{main}.
For most of the graphs, \mainalg{} was able to count all $k$-cliques in seconds or minutes.
For the largest {\tt com-orkut} graph, \mainalg{} ran in 1.5 hours. 
This is a huge improvement on the state of the art. For the ``infeasible"
instances in \Tab{main}, we do not get results even in two days using previous algorithms.
(This is consistent with results in Table 2 of~\cite{DBS18}, where some of the graphs are also
listed as ``very large graphs" for which clique counting is hard.)

A notable hard instance is {\tt com-lj} where \mainalg{} is unable to get all
clique counts in a day. Again, previous work also notes this challenge,
and only gives counts of $7$-cliques. We can get some partial results for {\tt com-lj},
as explained later.

% 
% , except the orkut graph which took about 1.5 hours, as shown in column ``time k''. Columns ``time V'' and ``time E'' are the time required to obtain the per-vertex and per-edge $k-$clique counts, resp. Note that the search tree for all cases is the same - the only difference is in the overhead of extra loops and data structure processing at every leaf. Even though it adds some time, it is still within a small factor of the time to count all $k$-cliques. Note that these timings are several orders of magnitude faster than the state-of-the-art, as we will show in the next section.

\begin{table*}[t]
\centering
% \caption{Graph properties}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Graph}         & \textbf{Vertices}     & \textbf{Edges}      & \textbf{Degen}  & \textbf{Max clique}
& \multicolumn{1}{|p{1.2cm}|}{\centering \mainalg{} \\ {\bf ($C_k$)}}
& \multicolumn{1}{|p{1.4cm}|}{\centering \mainalg{} \\ {\bf ($c_k(v)$)}}
& \multicolumn{1}{|p{1.4cm}|}{\centering \mainalg{} \\ {\bf ($c_k(e)$)}}
& \multicolumn{1}{|p{1.2cm}|}{\centering \mainalg{} \\ {\bf ($C_k$ parallel)}} \\
\hline
\multicolumn{9}{|c|}{Feasible by previous algorithms} \\
\hline
dblp-v5 & 1.56E+06 & 2.08E+06 & 15 & 10 & 7 & 7 & 8 & 19 \\
dblp-v7 & 3.67E+06 & 4.18E+06 & 19 & 12 & 15 & 16 & 19 & 34 \\
% dblp & 3.17E+05 & 1.04E+06 & 113 & 114 & 2 & 2 & 3 & 3 \\
amazon0601 & 4.03E+05  &  2.44E+06   & 10  &11&  4  & 5  & 6 & 4 \\
web-Google & 8.76E+05  &  4.32E+06   & 44 & 44 & 8 & 9 &15 & 9\\
youtube &1.13E+06   & 2.99E+06  &  51  &17  &7 & 8  &11 & 9 \\
cit-Patents &3.77E+06    &1.65E+07   & 64 & 11 & 40  &41 & 53 & 46 \\
soc-pokec  & 1.63E+06  &  2.23E+07  &  47 & 29 & 68& 75 &93 & 44 \\
\hline
\multicolumn{9}{|c|}{Not feasible for previous algorithms} \\
\hline
Stanford  &  2.82E+05   & 1.99E+06  &  71 &  61 & 5 &  5 & 38 & 3 \\
BerkStan  &  6.85E+05  &  6.65E+06   & 201 &201 &25 & 26  &237  & 9\\
as-skitter  & 1.70E+06   & 1.11E+07 &   111 & 67  & 120 & 200 &9245  & 75\\
com-orkut  & 3.07E+06  &  1.17E+08  &  253 & 51 & 5174   & 8802  & 99389  & 3441 \\ \hline
com-lj  & 4.00E+06  &  3.47E+07  &  360 & - & -   & -  & -  & 108000* \\ %6.4/42.5 hrs
% com-lj  & 4.00E+06  &  3.47E+07  &  360 & - & -   & -  & -  & 4029/7355* \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Table shows the sizes, degeneracy, maximum clique size, and the time taken (in seconds) by \mainalg{} to obtain global $k-$clique counts, per-vertex and per edge $k-$cliques counts for all k. *For the com-lj graph, we were not able to get all $k-$clique counts in 1 day so we tested for the maximum $k$ we could count in about a day. \mainalg{} was able to count the number of 9-cliques in 30 hours whereas kClist40 had not terminated even after 6 days.}
\label{tab:main}
\end{table*}


\begin{table}[]
\centering
% \caption{Comparison}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|r|r|r|}
\hline
\textbf{Graph}         & \textbf{k=13,TS}   & \textbf{k=13, kClist40}  & \textbf{all $k$, \mainalg{}} \\ %\cline{7-7}
\hline
Stanford  & 230 & 12600 &5 \\ %210
BerkStan  & 1198 &   > 172800 &25 \\ %1055 2 days
as-skitter & 798 & 12480 &120 \\ %715
com-orkut  & > 28800 &  > 172800  &5174\\ %36902 days
\hline
\end{tabular}
\end{adjustbox}
\caption{Time taken in seconds by the state-of-the-art randomized (TS, short for Tur\'anShadow) and parallel (kClist40) algorithms. Note that \mainalg{} obtains \textbf{all} $k-$clique counts for these graphs in a fraction of the time taken by other methods to count just 13-cliques.} 
\label{tab:comparison}
\end{table}



\begin{table}[]
\centering
% \caption{Comparison}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|r|r|r|}
\hline
\textbf{k}          & \textbf{$k$-cliques} &  \textbf{kClist40}  & \textbf{\mainalg{}} \\ %\cline{7-7}
\hline
7 & 4.49E+15 & 2.2 hours & 1.2 hours \\
8  & 1.69E+16 & 42.5 hours & 6.4 hours \\ %210
9 &  5.87E+17 & > 6 days & 30 hours \\ %715
10  & 1.89E+19 & > 6 days & 5.9 days \\ %3690
\hline
\end{tabular}
\end{adjustbox}
\caption{Table shows the time taken to count $k$-cliques for com-lj graph. For $k$=9, \mainalg{} terminated in about 30 hours where kClist40 had not terminated in 6 days.} 
\label{tab:com-lj}
\end{table}


\begin{figure*}[t!]
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/nCalls_vs_m.pdf}
        \caption{Number of nodes in SCT vs m}
        \label{fig:treesize}
    \end{subfigure}
~
\begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/trends.pdf}
    \caption{Trends in different graphs}
    \label{fig:trends}
    \end{subfigure}
~
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/trends-dblp.pdf}{}
    \caption{Trends in dblp over time.}
    \label{fig:trends-dblp}
    \end{subfigure}
     
\caption{\Fig{treesize} shows the number of nodes in the SCT vs the number of edges (m) for different graphs. The running time of \mainalg{} is directly proportional to the SCT size which seems to be roughly linear in the number of edges. \Fig{trends} shows the trends in clique counts for a number of graphs. For some of the graphs, the complete distribution of their clique counts has been obtained for the first time. \Fig{trends-dblp} shows the trends in the clique counts of 2 different versions over time of the dblp graph. }

\end{figure*}

% \begin{table*}[t]
% \centering
% % \caption{Graph properties}
% \label{tab:com-lj}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{|l|l|}
% \hline
% \textbf{Property}         & \textbf{value}     \\ 
% \hline
% vertices & 4.00E+06 \\
% edges & 3.47E+07 \\
% degeneracy & 360 \\
% k & 7 \\
% kClist40 & 7355 sec \\
% parallel \mainalg{} & 4029 sec \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison of timings for com-lj graph.} 
% \end{table*}

\textbf{Feasible local counting:} Notably, \mainalg{} can get per-vertex
counts in less than twice the time of global clique counting. Thus, we get 
results for more graphs in a few minutes, and can process the {\tt com-orkut}
graph within 3 hours. We consider this a significant achievement, given
the combinatorial explosion of clique counting.

\mainalg{} is also able to get per-edge clique counts, though
it can take an order of magnitude more time than global clique counting. Note that for obtaining the per-vertex and per-edge $k-$clique counts, the result data structure can become extremely large. Indeed, most of the time is spent in updating the data structure, rather than in constructing the SCT.
Nonetheless, for all but the {\tt as-skitter} and {\tt com-orkut} graph,
it runs in minutes. 

\textbf{Comparison with state of the art:} We only focus on the ``infeasible"
instances of \Tab{main}. For all the other instances, both \mainalg{} and kClist40
get results within two minutes. For space considerations, we do not report all
the running times for such instances. It is worth noting that the sequential
\mainalg{} is comparable to the parallel kClist40 (when they both terminate).

In \Tab{comparison}, we report times on TS and kClist40 on the hard datasets.
We are unable to get all values of $C_k$ using either of these two method. We run
these algorithms for up to 100 times the running time of \mainalg{} or two days, whichever
is shorter. We try to count the largest feasible clique count.

Let us focus on kClist40, where we cannot go beyond counting 13-cliques
(we note that this is consistent with results reported in~\cite{DBS18}). 
Notably, in the {\tt BerkStan} graph, kClist40 needs more than 2 days to count
13-cliques, while \mainalg{} gets all clique counts in a minute. As mentioned
earlier, clique counting on the large {\tt com-orkut} graph is done in a few
hours by \mainalg, while even counting 13-cliques takes kClist40 more than two days.

TS also does not scale well for larger cliques and \mainalg{} is faster than TS. For example, for the {\tt Stanford} graph, TS required 230 seconds to estimate the number of 13-cliques whereas \mainalg{} obtained all $k-$clique counts in 5 seconds. Similar trends are observed with other graphs. 

% , which
% can only count 10 cliques approximately. 
% The only instance where TS is faster is for {\tt com-orkut}, but again,
% we stress that TS cannot count larger cliques.

% \textbf{TS:} This is an approximate clique counting algorithm for $k$ upto 10. It mines dense subgraphs (shadow) and samples cliques within the dense subgraphs to give an estimate. It requires the entire shadow to be available for sampling which can require considerable space. 
% 
% \textbf{kClist40:} This algorithm by Danisch et. al. ~\cite{Danisch18} uses ordering and parallelization to enumerate all cliques. Note however that in the implementation provided by the authors, they do not list every clique but simply update the count of $k-$cliques. Although the algorithm in principle can provide per-vertex and per-edge $k-$clique counts, the algorithm would run into the same problem as we did in the parallelization of \mainalg{}, namely that the replication of result data structures can take up a lot of memory. Hence, we feel the right comparison of kClist with \mainalg{} should be with the parallel version of \mainalg{} that simply counts all $k-$cliques. 
% 
% The authors also do a detailed study of the runtimes of the Chiba-Nishizeki algorithm ~\cite{ChNi85} (on which their clique enumeration algorithm is based), the sequential version of their algorithm (kClist) and 2 parallel versions kClistNodeParallel and kClistEdgeParallel. The authors show that out of all the different variants they experimented with, kClistEdgeParallel with 40 threads (abbreviated to kClist40) gives the best performance and we will use this for comparison. Note that  kClist40 is the only algorithm that attempts to count cliques beyond size 10 that does not require Map-Reduce or any specialized hardware. The algorithm lists every clique. Thus, when it encounters a clique, it enumerates every smaller clique contained inside it. For the purpose of counting, this is wasteful as one could simply get the number of smaller cliques contained inside a clique by calculating ${n \choose k}$ where $n$ is the size of the clique and $k<n$ is the size of smaller clique. So we optimize their algorithm and indeed, in some cases we see significant improvement in the running time. For any results listed for kClist40 in this paper we use this optimization. Note that \mainalg{} algorithm can easily be used for listing all cliques, however we consider that out of the scope of this paper and focus on counting. 
% 
% \textbf{Runtime comparison:} \Tab{comparison} shows the running times of the 3 algorithms and their comparison with \mainalg{}. For $k=5$, all algorithms terminate in seconds for most graphs. At $k=10$, the difference in runtimes starts showing and while approximate counting still works in seconds in most cases, exact counting slows down significantly. At $k=13$, the only available option, did not terminate after several days for many of the graphs. \mainalg{} not only terminated in seconds and minutes, but gave counts of \textit{all} $k-$cliques. For $k=13$ we obtain a speedup of several orders of magnitude. As $k$ increases further (the largest clique size we encountered in the graphs we experimented with was 201), the number of $k$-cliques goes up expenentially and enumeration is bound to perform extremely poorly) Indeed, in some cases it might even be impossible to enumerate all cliques. This clearly indicates the advantage that counting has over enumerating. 

\textbf{Parallel global clique counting:} As mentioned in \Sec{count}, we do a simple
parallelization of the global clique counting of \mainalg{} using 30 threads. It gives moderate benefits
for most instances, and about a factor two speedup for large instances.
For the challenging {\tt com-lj} instances, the effect is much more dramatic. 
We are able to count $7$-cliques in an hour using the parallel \mainalg, while
the sequential version takes more than a day.

\textbf{Performance on com-lj.} This is a particularly challenging graph. 
The sequential version of \mainalg{} for counting all $k$-cliques did not terminate within a day, 
so we used the parallel version of our algorithm to show a comparison for global
counts upto $k=10$. We can truncate the SCT to get cliques of some fixed size.
\Tab{com-lj} shows the results. Even for this graph, the parallel version of \mainalg{} is faster than kClist40 for $k=7$ and beyond. kClist40 did not terminate after six days,
for $k = 9$ and beyond. We note the astronomical number
of 10-cliques ($> 10^{19}$), which makes enumeration infeasible, but \mainalg{}
was able to get the exact count.

% For $k=8,9,10$, \mainalg{} took 6.4, 30 and 142 hours respectively, whereas kClist40 required 42.5 hours for $k=8$, and for $k=9$ and $10$, the algorithm had not terminated even after 6 days. The counts of these $k-$cliques is 1.69E+16, 5.87E+17 and 1.89E+19, respectively. Considering the increasing trend and the large count of $k-$cliques for $k=8,9$ and $10$, obtaining clique counts for larger $k$ would be \Shweta{near-impossible} using other methods.

\textbf{Size of $\sct(G)$:} In \Fig{treesize}, we plot
the number of nodes of $\sct(G)$ as a function of the number
of edges in $G$. We observe that for most graphs, the size
is quite close to $m$, explaining why \mainalg{} is efficient.

% Since the tree generated by \mainalg{} is much smaller than the tree generated by kClist40, we suspect this trend will continue.

 % using the parallel version of our algorithm 

% As the both of \mainalg{} and kClist40} for the sequential algorithm ran into days, 

% \Shweta{Note that maximal clique counting algorithm of Eppstein did not terminate on the 2 graphs even in days so it is not unexpected that our's won't either. The caveat is that Max's algorithm can be used to count for small k on those graphs using parallelization. We can also do it for small k (7) and in time somewhat less than what their algo takes. But their algo with the above mentioned optimization takes lesser time than our algorithm. I think this means that there is still a case for parallelization and perhaps we should mention it that way. }
% \Shweta{Update: Parallel algorithm is running. Hopefully will have numbers soon. The drawback of our algorithm that to count k-cliques, it needs to build the tree to depth much more than k, and hence takes more time, is still there. But for bigger k, our algorithm definitely gives an advantage.}

% \begin{table*}[]
% \centering
% % \caption{Comparison}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{|l|l|l|r|r|r|r|r|r|}
% \hline
% \textbf{graph}         & \textbf{k=5, Escape}     & \textbf{k=5,kClist40}      & \textbf{k=5,TS}  & \textbf{k=10, kClist40}        & \textbf{k=10,TS}   & \textbf{k=13, kClist40}  & \textbf{ECC} & \textbf{ECC parallel}\\ %\cline{7-7}
% \hline
% amazon0601 & 1 &   2  & 2  & 2 &  2  & 2 & 4 & 4\\
% cit-Patents &4 &  10 & 15& 10 & 14 & 10 &40 & 46 \\
% web-Google & 4 &  2  & 3 &  2 & 3  & 2 &8 & 9\\
% soc-pokec  & 20 & 10 & 108 &11 &  110 & 11 &68 & 44\\
% youtube & 2 &  2 &  21 & 2 &  25&  2 &7 & 9\\
% Stanford  &  18 & 2  & 77 & 182 &   210 & 12600 &5 & 3\\
% BerkStan  &  902 & 4 &  405 & >235800 &  1055 &   >235800 &25 & 9\\
% as-skitter  & 74 & 5 &  618 &244   & 715 & 12480 &120 & 75\\
% com-orkut  & 1924  &  57 & 1236  &  7261 &  3690 &  280020 &5174 & 3441\\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Table shows the time taken by the parallel clique listing algorithm kClist with 40 threads for different $k$, time taken by Escape to count 5 cliques, and time taken by Tur\'anShadow for counting 5 and 10 cliques. As $k$ increases, the time taken by these algorithms blows up. \mainalg{} on the other hand obtains counts of \textbf{all} cliques in of fraction time taken by other algorithms, thus giving a speedup of several orders of magnitude. The parallel version of \mainalg{} gives a further speedup, esp. for large graphs (for smaller graphs, the overhead of parallelization masks the savings in run-time due to parallel processing.)} 
% \label{tab:comparison}
% \end{table*}
% 

    % \caption{\footnotesize{Figure shows a plot of the number of $k-$clique counts in several real world graphs. The largest clique encountered was of size 201. The largest $k$ for which state of the art methods have been able to obtain $k-$clique counts for is 29 ~\cite{DBS18}. This complete picture of the trends in $k-$clique counts has been obtained for the first time for these graphs.}} 
    %     \label{fig:dblp}

% \begin{figure*}[t!]
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/nCalls_vs_m.pdf}
%         \caption{\footnotesize{nCalls vs m}}
%         \label{fig:nCalls-vs-m}
%     \end{subfigure}
% ~
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/sumP_vs_m.pdf}
%         \caption{\footnotesize{sumP vs m}}
%         \label{fig:sumP-vs-m}
%     \end{subfigure}
% ~
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/sqP_vs_m.pdf}
%         \caption{\footnotesize{sqP vs m}}
%         \label{fig:sqP-vs-m}
%     \end{subfigure}
%     \caption{Comparison of nCalls, sumP and sqP with m. nCalls seems to scale roughly linearly with m.}
% \end{figure*}

% \begin{figure*}[t]
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/nCalls_vs_time.pdf}
%         \caption{\footnotesize{Timings}}
%         \label{fig:nCalls-vs-time}
%     \end{subfigure}
% ~
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/sumP_vs_time.pdf}
%         \caption{\footnotesize{Runtime comparison with other algorithms}}
%         \label{fig:sumP-vs-time}
%     \end{subfigure}
% ~
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/sqP_vs_time.pdf}
%         \caption{\footnotesize{Number of recursive calls}}
%         \label{fig:sqP-vs-time}
%     \end{subfigure}
%     \caption{ Comparison of nCalls, sumP and sqP with time.}
% \end{figure*}


% \Shweta{To include: Table of graph stats, time required to count all $k-$cliques by \mainalg{} and also time to obtain per-vertex and per-edge counts using \mainalg{}. Also, time required by other methods - Max's, TS, ESCAPE, MapReduce(?) to count 5, 7, 10 cliques for these graphs. We need to think of whether we want to include the results of MapReduce or not.}

% \Shweta{Timings for David's max clique finding algorithm are very less because they use aggressive branch and bound techniques, so comparison with their algorithm may not be fruitful.}

% \subsection{Properties of the recursion tree} \label{sec:tree}

% The main advantage that \mainalg{} has over the clique enumeration algorithm of ~\cite{ChNi85} and ~\cite{Danisch18} is in the reduced size of the search tree. We define several parameters to analyze the behaviour of the algorithm. $nCalls$ indicates the number of recursive calls made by the algorithm, $sumP$ indicates the sum of the sizes of the $P$ (number of vertices) set obtained at each recursive call, and $sqP$ indicates the sum of the square of the sizes of the $P$ (number of vertices) set obtained at each recursive call. The size of the search tree can be seen to be roughly proportional to the runtime of the algorithm. But more importantly, there difference between $nCalls$, $sumP$ and $sqP$ is not very large, indicating that the $P$ for most of the recursize calls is not very large. 

\subsection{Demonstrations of \mainalg} \label{sec:appl}

Global and local cliques have numerous applications. It is 
outside the scope of this work for detailed demonstrations, but
we show a few examples in this section.

As mentioned earlier, local clique counts are an important aspect
of graph processing. In \Fig{soc-pokec-occurrences} and \Fig{web-Stanford-occurrences}, we plot the per-vertex
clique distributions, also called the \emph{graphlet} degree
distribution in bioinformatics~\cite{Pr07} for the as-skitter and web-Stanford graphs. We choose values
of $k = 5, 10, 15, 20, 25$. Then, we plot the function $f_k(b)$
that is the number of vertices that participate in $b$ $k$-cliques.
We notice interesting trends. While the as-skitter graph
has a nicely decaying $f_k$ function, there is much more noise
in web-Stanford. It would be interesting to design models
that can capture such behavior in the local clique counts.

% {\tt dblp} {\tt com-youtube}

In \Fig{trends}, we plot the $C_k$ values for a number of graphs.
We notice, for example, that the {\tt soc-pokec} network has a ``flatter" distribution of $C_k$ for some of the initial values,
while the {\tt com-orkut} graph looks much closer to a binomial distribution. The latter suggests that the bulk of cliques are coming
from the maximum clique in the {\tt com-orkut} graph, but not
so in the {\tt soc-pokec} graph.

In \Fig{trends-dblp}, we plot the $k$-clique counts (vs $k$)
for two different versions across time for the DBLP citation network~\cite{Aminer}. 
Interestingly, despite the later version only having less than twice as many edges, 
the clique distribution (plotted in semilog) has a much bigger difference. It appears
that the graph is becoming significantly dense in certain part.
This sort of analysis may help in understanding dynamic graphs. 

% \begin{figure}[t]
%     \begin{subfigure}[b]{0.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/trends.pdf}
%     \end{subfigure}
%     \caption{\footnotesize{Figure shows a plot of the number of $k-$clique counts in several real world graphs. The largest clique encountered was of size 201. The largest $k$ for which state of the art methods have been able to obtain $k-$clique counts for is 29 ~\cite{DBS18}. This complete picture of the trends in $k-$clique counts has been obtained for the first time for these graphs.}} 
%     \label{fig:trends}

% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/trends-dblp.pdf}{}
%         % \caption{\footnotesize{Trends in dblp over 3 versions.}}

% % \vfill
% % \begin{subfigure}[]{0.22\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{Figures/sumP-vs-m.pdf}
% %         % \caption{\footnotesize{sumP vs m}}
% %         \label{fig:sumP-vs-m}
% %     \end{subfigure}
% % ~
% % \begin{subfigure}[]{0.22\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{Figures/sqP-vs-m.pdf}
% %         % \caption{\footnotesize{sqP vs m}}
% %         \label{fig:sqP-vs-m}
% %     \end{subfigure}
% \caption{\footnotesize{Trends in the clique counts of 2 different versions over time of the dblp graph. \Shweta{Not sure what more to write here.}}}
%         \label{fig:dblp}
% \end{figure}

% 
% We obtained version 5 of citation network formed by a crawl of DBLP from ~\cite{DBLP}. We discovered the vertex that participated in the
% maximum number 
% 
% The edge (pair of publications) that participates in most cliques is ``Interactive control of avatars animated with human motion data.'' and ``Motion graphs.'' and it participates in 15595 $k-$cliques. The vertex (publication) that participates in most cliques is ``R-Trees: A Dynamic Index Structure for Spatial Searching'' and it participates in 13441 cliques. The average number of cliques that any vertex is involved in is 9.7. Average size of clique that a vertex is involved in is 3.24. The largest clique was of size 12 and there were 3 such cliques. Publications forming these cliques are given in \Tab{papers}.


% \subsection{Trends in clique counts of real world graphs} \label{sec:trends}
% Before this work, for a lot of the graphs, clique counts for only small $k$ were known. Because \mainalg{} obtains all clique counts in a fraction of the time of other algorithms, for the first time, we are able to observe the trends in clique counts across all $k$ for these graphs. \Fig{trends} shows the plot of the exact number of $k-$clique counts in many of these graphs. It is interesting to observe that there is quite a lot of variation in the size of the largest clique. Moreover, the binomial-like shape of the curve is indicative of the existence of a few large cliques which supply the bulk of the smaller cliques. It would be interesting to see how the incorporation of these observed trends in graph generation models improve the similarity of the graphs generated with graphs found in reality. 
% 
% 

% \begin{table}[] \label{tab:dblp}
% \centering
% % \caption{DBLP}
% \begin{adjustbox}{max width=0.45\textwidth}
% \begin{tabular}{|r|r|}
% \hline
% \textbf{k}         & \textbf{Ck} \\ 
% \hline
% 0 &  1 \\
% 1 &  3677950 \\
% 2 &  4187388 \\
% 3 &  3292029 \\
% 4 &  1785122 \\
% 5 &  800541 \\
% 6 &  304338 \\
% 7 &  96001 \\
% 8 &  24241 \\
% 9 &  4726 \\
% 10 &  672 \\
% 11 &  63 \\
% 12 &  3 \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Table shows the number of k-cliques in the DBLP graph (version 5).} 
% \end{table}
% \begin{table*}[] \label{tab:papers}
% \centering
% % \caption{DBLP}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{|l|}
% \hline
% \textbf{title}     \\ 
% \hline
% Clique 1 \\
% \hline
% Formal verification of superscale microprocessors with multicycle functional units, exception, and branch prediction. \\
% Optimization of the DET curve in speaker verification. \\
% Effective use of Boolean satisfiability procedures in the formal verification of superscalar and VLIW microprocessors. \\
% Automatic formal verification of reconfigurable DSPs. \\
% Exploiting Signal Unobservability for Efficient Translation to CNF in Formal  \\
% Processor verification using efficient reductions of the logic of uninterpreted functions to propositional logic. \\
% Automatic verification of Pipelined Microprocessor Control. \\
% Efficient translation of boolean formulas to CNF in formal verification of microprocessors. \\
% Method for Formal Verification of Soft-Error Tolerance Mechanisms in Pipelined Microprocessors. \\
% Exploiting Abstraction for Efficient Formal Verification of DSPs with Arrays of Reconfigurable Functional Units. \\
% Techniques for Verifying Superscalar Microprocessors. \\
% A method for debugging of pipelined processors in formal verification by correspondence checking. \\
% \hline
% Clique 2 \\
% \hline
% Formal verification of superscale microprocessors with multicycle functional units, exception, and branch prediction. \\
% Using Abstraction for Efficient Formal Verification of Pipelined Processors with Value Prediction. \\
% Automatic Abstraction of Memories in the Formal Verification of Superscalar Microprocessors. \\
% Effective use of Boolean satisfiability procedures in the formal verification of superscalar and VLIW microprocessors. \\
% Automatic formal verification of reconfigurable DSPs. \\
% Exploiting Signal Unobservability for Efficient Translation to CNF in Formal Verification of Microprocessors. \\
% Processor verification using efficient reductions of the logic of uninterpreted functions to propositional logic. \\
% Automatic verification of Pipelined Microprocessor Control. \\
% Efficient translation of boolean formulas to CNF in formal verification of microprocessors. \\
% Method for Formal Verification of Soft-Error Tolerance Mechanisms in Pipelined Microprocessors. \\
% Exploiting Abstraction for Efficient Formal Verification of DSPs with Arrays of Reconfigurable Functional Units. \\
% Techniques for Verifying Superscalar Microprocessors. \\
% \hline
% Clique 3 \\
% \hline
% Seamless Implementation of a Telephone Switching System Based on Formal Specifications in RTPA. \\
% Design and Implementation of an Autonomic Code Generator Based on RTPA. \\
% The Formal Design Model of an Automatic Teller Machine (ATM). \\
% On Contemporary Denotational Mathematics for Computational Intelligence. \\
% The Formal Design Models of a Set of Abstract Data Types (ADTs). \\
% The Formal Design Models of Tree Architectures and Behaviors. \\
% The Formal Design Models of a Universal Array (UA) and its Implementation. \\
% The Formal Design Model of Doubly-Linked-Circular Lists (DLC-Lists). \\
% The Formal Design Model of a Real-Time Operating System (RTOS+): Static and Dynamic Behaviors. \\
% The Formal Design Model of a File Management System (FMS). \\
% The Formal Design Model of a Real-Time Operating System (RTOS+): Conceptual and Architectural Frameworks. \\
% The Real-Time Process Algebra (RTPA). \\
% \end{tabular}
% \end{adjustbox}
% \caption{Table shows the 3 cliques of size 12 in the dblp graph.} 
% \end{table*}

%     \begin{figure}[t!]
%     \begin{subfigure}[]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/publications-references_occurrences.pdf}{}
%         \label{fig:dblp-occurrences}
%     \end{subfigure}
%     % \end{figure}
% ~
%     % \begin{figure}
%      \begin{subfigure}[]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/web-Stanford_occurrences.pdf}{}
%         \label{fig:amazon-occurrences}
%     \end{subfigure}
%     % \end{figure}
% \vfill
%     % \begin{figure}
%      \begin{subfigure}[]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/com-youtube_occurrences.pdf}{}
%         \label{fig:amazon-occurrences}
%     \end{subfigure}
%     % \end{figure}
% ~
%     % \begin{figure}
%     \begin{subfigure}[]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/web-Google_occurrences.pdf}{}
%         % 
%         \label{fig:amazon-occurrences}
%     \end{subfigure}

% \caption{\footnotesize{Figure shows the $k$-clique distribution for k=5, 8 and 12 for different graphs. These counts are useful in graph generation and analysis. \Shweta{check caption please.}
%     }\label{fig:occur}}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/nCalls-vs-m.pdf}
%         % \caption{\footnotesize{nCalls vs m}}
% % \vfill
% % \begin{subfigure}[]{0.22\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{Figures/sumP-vs-m.pdf}
% %         % \caption{\footnotesize{sumP vs m}}
% %         \label{fig:sumP-vs-m}
% %     \end{subfigure}
% % ~
% % \begin{subfigure}[]{0.22\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{Figures/sqP-vs-m.pdf}
% %         % \caption{\footnotesize{sqP vs m}}
% %         \label{fig:sqP-vs-m}
% %     \end{subfigure}
% \caption{\footnotesize{Size of the SCR tree (also the number of recursive calls made) for different graphs as a function of the number of edges $m$. The size of the tree is roughly linear in $m$.}}
%         \label{fig:treesize}
% \end{figure}



\section{Future work} \label{sec:future}

We provide an exact clique counting algorithm that counts all $k$-cliques in a fraction of the time of other state-of-the-art parallel algorithms. One of the key ideas is the use of pivoting to create
the SCT, and succinct representation of all the cliques of the
graph. The success of~\cite{DBS18} in using parallelization
for clique counting suggests combining their ideas with our pivoting
techniques. We may be able to come up with an efficient parallel
building of the SCT that is much faster than our current implementation. Indeed, the results on the {\tt com-lj} graph suggest
that even \mainalg{} has its limits for real data.

An orthogonal approach would be to exploit the sampling techniques
in the Tur\'{a}n-Shadow algorithm~\cite{JS17}. For many subgraph
counting problems, randomization has been the key to truly practical
algorithms. We believe that \mainalg{} could be made faster with 
these ideas.


Moreover, it also gives per-edge and per-vertex $k-$clique counts. This is the first time that $k-$clique counts are known for many of the graphs we experimented with and this will open doors for further use of cliques in generation and analysis of graphs.



